Task-Customized Mixture of Adapters for General Image Fusion

General image fusion aims at integrating important information from multi-source images. However, due to the significant cross-task gap, the respective fusion mechanism varies considerably in practice, resulting in limited performance across subtasks. To handle this problem, we propose a novel task-customized mixture of adapters (TC-MoA) for general image fusion, adaptively prompting various fusion tasks in a unified model. We borrow the insight from the mixture of experts (MoE), taking the experts as efficient tuning adapters to prompt a pre-trained foundation model. These adapters are shared across different tasks and constrained by mutual information regularization, ensuring compatibility with different tasks while complementarity for multi-source images. The task-specific routing networks customize these adapters to extract task-specific information from different sources with dynamic dominant intensity, performing adaptive visual feature prompt fusion. Notably, our TC-MoA controls the dominant intensity bias for different fusion tasks, successfully unifying multiple fusion tasks in a single model. Extensive experiments show that TC-MoA outperforms the competing approaches in learning commonalities while retaining compatibility for general image fusion (multi-modal, multi-exposure, and multi-focus), and also demonstrating striking controllability on more generalization experiments. The code is available at https://github.com/YangSun22/TC-MoA .

==> sec/0_abstract.tex <==
\begin{abstract}
% Image fusion aims to obtain an image that aggregates important information from multiple source images captured by different sensors in the same scene. General image fusion methods are compatible to solve multiple image fusion tasks, including multi-modal, multi-focus and multi-exposure image fusion. 

% 不同的图像融合场景，任务需求不同，融合规则差异大，难以用统一的模型学习。

% 现有multi-source数据规模普遍较小,表达能力不足，影响性能->大模型->融合规则差异大，难以形成统一融合模型，考虑动态->MoA->Task-customized
%背景
% \cb{General image fusion aims at integrating important information from multi-source images. However, due to the significant cross-task gap, the respective fusion mechanisms vary considerably in practice, resulting in limited performance across subtasks.
% To handle this problem,  }
% 也可以直接从微调的角度入手
% Parametric efficient learning has been widely used in various vision tasks, but few efforts have been made in image fusion, even less in general fusion.
%现有的图像融合数据规模较小，导致网络特征的提取和表示能力不足，无法精确地感知并学习融合规则。因此我们使用自监督预训练的视觉大模型作为基础结构。
%Existing techniques usually tap into commonalities among different sources to perform general image fusion through a unified model.


    
%现有的通用融合任务通常为不同任务寻找共性，对不同任务使用统一的的框架和学习目标，学习不同融合规则的交集。然而，不同任务的融合规则差异很大，交集并不能很好地处理具体的单个任务。为了解决这个问题，我们提出了xxxx，
%我们的方法可以自适应地感知不同的融合任务中动态变化的模态主导强度
%通过主导强度实现动态兼容多种融合任务的统一图像融合框架
%prompt的平均主导强度反映了任务在token-level的融合规律。主导强度差反映了任务在source-level的规律。通过tc-moa动态定制prompt，从而间接动态调制融合规则。
%能够动态自适应兼容多个融合任务的统一图像融合框架
%突破多任务瓶颈
%基于prompt的主导强度反映了不同任务的融合规律, 
%我们提出一种新的统一融合框架，可以动态自适应兼容不同的融合任务by主导强度，保留任务个性，从而突破多任务共性的瓶颈。We borrow the insight from the mixture of experts (MoE), 设置了  adapter bank和router bank. adapter bank保管所有任务的融合模式，每个adapter代表一种融合模式。router bank 包含task-specific routers, 每个router作为一种任务偏置的查询可以定制mixture of adapter处理当前的样本，具体来说生成了prompt for fusion, 即在token-level的不同源对融合结果的主导强度。主导强度代表源信息在融合信息的比例。对融合结果的贡献程度。代表融合图像受源图像多大影响。代表源信息在融合信息的重要程度。不同源的主导强度由归一化/互补loss约束，保证信息是互补的

% 我们提出一种新的统一融合框架，named as TC-MoA, 可以动态自适应兼容不同的融合任务的个性, 从而突破多任务只学习共性的瓶颈。We borrow the insight from the mixture of experts (MoE), 在框架中设置了 adapter bank和task-specific router bank.
%adapter bank负责保管所有任务的融合模式，每个adapter负责记忆一种融合模式。router bank 的 每个router可以为当前样本定制任务偏置的mixture of adapters来生成prompt for fusion。prompt代表TC-MoA对每个源的含有重要信息占所有源的比例的估计 in patch-level.如果某个源的平均prompt值越大，就更在融合中占主导地位，即主导强度。我们通过动态地调制mixture of adapters动态估计主导强度。模型根据主导强度抽取相关信息生成融合图像。
% To handle this problem, we propose a novel task-customized mixture of adapters (TC-MoA) for general image fusion, jointly and adaptively compatible with various fusion tasks, 
% masters task-biased appetite for adapters to customize suit-085
% able mixture of adapters, and every shared adapter pos-086
% sesses a mechanism for generating the prompt.
\cb{General image fusion aims at integrating important information from multi-source images. However, due to the significant cross-task gap, the respective fusion mechanism varies considerably in practice, resulting in limited performance across subtasks. To handle this problem, we propose a novel task-customized mixture of adapters (TC-MoA) for general image fusion, adaptively prompting various fusion tasks in a unified model. We borrow the insight from the mixture of experts (MoE), taking the experts as efficient tuning adapters to prompt a pre-trained foundation model. 
These adapters are shared across different tasks and constrained by mutual information regularization, ensuring compatibility with different tasks while complementarity for multi-source images. The task-specific routing networks customize these adapters to extract task-specific information from different sources with dynamic dominant intensity, performing adaptive visual feature prompt fusion. Notably, our TC-MoA controls the dominant intensity bias for different fusion tasks, successfully unifying multiple fusion tasks in a single model. Extensive experiments show that TC-MoA outperforms the competing approaches in learning commonalities while retaining compatibility for general image fusion (multi-modal, multi-exposure, and multi-focus), and also demonstrating striking controllability on more generalization experiments. Our code will be released for more potential applications.}
% we propose a novel unified image fusion framework, named TC-MoA, which can dynamically adapt to and accommodate various fusion tasks, thereby breaking through the performance bottleneck of multi-task unified learning. We borrow the insight from the mixture of experts (MoE), and introduce the shared-adapters bank and task-specific routers' bank into our framework. Adapters memorizing different fusion patterns, while routers generate prompt for fusion by customizing a task-biased mixture of adapters with for the current sample. The prompt value, which represents the estimate of the proportion of important information contained in each source, is also referred to as the dominance intensity, indicating the level of dominance a particular source possesses. To guide the learning of dominant intensity of multi-source, we design a complementary loss.
% \cb{
% Extensive experiments demonstrate that TC-MoA outperforms the competing approaches in learning commonalities while retaining compatibility for general image fusion (multi-modal, multi-exposure, and multi-focus), showing superior fusion performance qualitatively and quantitatively.}
% % The prompt is the estimate of the proportion of important information contained in each source. The higher the prompt value for a particular source, the more dominant it is considered. Therefore, this value is referred to as the dominance strength. 







%TC-MoA consists of a explicit Task-driven feature Select/Pick Module and a Refine Module.After The a frozen pre-trained encoder extract features of multi-source images separately. The Select Module customize a fusion prompting and obtain fused features based on multi-source features by using Mixture of Adapters.According to Task-Customized prompting each Token of the multi-source feature is explicitly given the degree of contribution to the fused features. In order to ensure that the Select Module works properly and that there is physical meaning to the contribution values, we propose a complementary feature constraint. The fusion feature can be reintegrate and align to feature space of the pre-trained model by using the Refine Module.our model achieves far superior fusion performance in comparison with the general image fusion methods.Our code will be released for potential broader applications.


%Our model consists of a universal bi-directional adapter and multiple modality-specific transformer encoder branches with sharing parameters. The encoders extract features of each modality separately by using a frozen pre-trained foundation model. We develop a simple but effective light feature adapter to transfer modality-specific information from one modality to another, performing visual feature prompt fusion in an adaptive manner. With adding fewer (0.32M) trainable parameters, our model achieves superior tracking performance in comparison with both the full fine-tuning methods and the prompt learning-based methods. Our code will be released for potential broader applications.

%To our best knowledge, we first introduce the pretrained model to image fusion.

%TC-MoA consists of a multi-gated(task-specific gated) Mixture of Adapters(experts) and a Refine Module. 

% %--------- 1. 介绍Task-Customized、Mixture of Adapters---------------

% TC-MoA consists of an explicit Task-customized feature Select/Pick Module and a Refine Module.

% %After The a frozen pre-trained encoder extract features of each source image separately. 
% After The a frozen pre-trained encoder extract features of multi-source images separately. 
% %The encoders extract features of each source image separately by using a frozen pre-trained foundation model.

% The Select Module customize a fusion prompting and obtain fused features based on multi-source features by using Mixture of Adapters.

% %--------- 2. A+B=1 的显式的融合结构和Loss---------------------------

% %Fusion prompting is expressed based on Mixture of Adapters
% %According to Task-Customized prompting Each Token of the multi-source feature specifies its contribution to the fused image.
% According to Task-Customized prompting each Token of the multi-source feature is explicitly given the degree of contribution to the fused features. In order to ensure that the Select Module works properly and that there is physical meaning to the contribution values, we propose a complementary feature constraint. 

% %--------- 3. Refine（可选）------------------------------------

% The fusion feature can be reintegrate and align to feature space of the pre-trained model by using the Refine Module.

% 4. ---------性能---------------------------------------------

% our model achieves far superior fusion performance in comparison with the general image fusion methods.

% 5.--------- 开源---------------------------------------------

% Our code will be released for potential broader applications.



% Due to the limited data scale of paired multi-source data, the capability of feature representation of the network is not fully developed to recognize the fusion guidelines accurately. Therefore we use a self-supervised pre-trained vision model as the backbone.
%%同时，由于不同的图像融合任务的源图像物理意义不同，融合规则差异大，难以用统一的模型学习。因此我们使用任务定制的通用图像融合Adapters。
% Meanwhile, the image fusion tasks have different physical meanings of multi-source images, resulting in widely varying fusion guidelines that are tricky to learn with a unified model. 
%To handle this problem, we propose a Task-Customized Mixture of Adapters for General Image Fusion. 

%首先，为了兼容不同任务的融合目标，MoAFusion引入了一个多门控的MoAdapter。门控网络是任务特定的，这允许模型根据任务定制不同的Adapter混合。

%Firstly, to be compatible with the fusion guidelines, We introduces a multi-gated Mixture of Adapters(experts). The gating networks are task-specific, which allow to customize the mixture of Adapters(experts) according to the task.

%然后，为了指导MoA稳定地学习融合规则s，我们引入了用于显式地评估信息保留的Attention网络结构，对于Multi-source的每个token任务导向地评估其信息在融合特征中的保留程度。

%Then, to guide MoA to learn fusion guidelines stably, we design modules for explicit information retention evaluation based on attention, for each token of Multi-source images evaluating the importance in the fusion features task-orientedly.


%最后，为了使融合特征保持在大模型的特征空间内，我们使用Refine Module，重新修饰了融合特征。
%Finally, in order to keep the fusion features within the feature space of the pre-trained model, we use the Refine Module to reintegrate and align.


%大量的实验表明，我们的网络可以根据样本输入不同提供任务定制的融合规则，并且获得SOTA。
%Extensive experiments show that our network can provide task-customized fusion guidelines and obtain SOTA.


%usually use the same network and loss function, which misses the differences between tasks and leads to compromised learning. 
%In this paper, we propose a novel unsupervised general image fusion approach, called AIAFusion, which can adaptively customize a fusion plan for each sample. First, an MoE-based Attention in Attention module is introduced to achieve adaptive fusion of various samples for different tasks. The shared experts in the module are utilized to preserve the commonalities, and the task-specific gating network is utilized to bring out the individuality. Then, to instruct the AIA module to learn how to trade off information from different sources, an information complementarity constraint is introduced. Finally, a module of feature refined is added to align the feature space of the frozen self-supervised pre-trained model, which brings excellent feature extraction and reconstruction capabilities. Extensive experiments show that on multiple fusion tasks, our approach successfully preserves the individuality of the task and obtains SOTA.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}




\begin{figure}
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  \includegraphics[width=\linewidth]{img/TC-MoA_11_14_Introduction.pdf}
  \vskip -0.1in
   \caption{Prompt can adaptively select the complementary information from multi-source features. The dominant intensity bias vary according to the task, which is reflected by the different shades of colors.}
   \label{fig:introduction}
    \vspace{-1.8em} 
\end{figure}



% \begin{figure}[ht]
%     \includegraphics[width=1\linewidth]{img/TC-MoA_11_14_Introduction.pdf}\captionsetup{skip=0pt} 
%     \vspace{-1.3em}
%     %\vskip 1in
     
%   \caption{Prompt can adaptively select the complementary information from multi-source features. The dominant intensity biases vary according to the task, which is reflected by the different shades of color.}
%    \captionsetup{skip=0pt} 
%   \label{fig:introduction}
%   \vspace{-0.7em}
% \end{figure}



% 多模态统一图像融合框架 + Adapter  + MMoE
% Framework/Paradigm/Method
% Pick-and-Fit / Pick-and-Refine
% Attention in Attention
% Mixture-of-Experts
% Multi-Task

% A general image fusion framework via a dynamic Pick-and-Refine adapter based on Attention in Attention Mixture-of-Experts.

% A Pick-and-Refine adapter by using Attention in Attention for general image fusion

% Learning to notice \{preserve\} individuality: An Attention in Attention Mixture-of-Experts adapter for general image fusion

% Mixture of Attention in Attention for General Image Fusion

% Mixture of Task-Customized Adapters for General Image Fusion

% Mixture of Task-Customized Experts for General Image Fusion
% Adapter-oriented Mixture of Task-Customized Experts for General Image Fusion
% Mixture of Task-Customized Adapters for General Image Fusion
% Task-Customized Adapters for General Image Fusion

% Fusion from Decomposition: A Self-Supervised
% Decomposition Approach for Image Fusion

% IFCNN: A general image fusion framework based on convolutional neural network

% Task-specific(task customized) Attention Adapter for General Image Fusion

% A general image fusion framework based on task-specific Attention

% Mixture-of-Experts in Attention 
Image fusion aims to integrate complementary information from multi-source images captured by different sensors in the same scene onto a single image. It is usually used to enhance important information and visual quality \cite{IF_Survey,IF_DL_Survey}.
Currently, general image fusion mainly includes multi-modal, multi-exposure, and multi-focus image fusion, \etc 
The \textit{Multi-Exposure image Fusion} (MEF) focuses on integrating images with multiple exposure levels into a high-quality full exposure image~\cite{MEF_Survey}. 
% 有引用支撑吗？？
% 不知道算不算，MEF-Net原文:Research in MEF has yielded a number of methods [2]–[8], which generate fused images with faithful detail preservation and vivid color appearance. This is mainly accomplished by a weighted summation framework.
Each source image contributes its own illumination and structural information to the fused image~\cite{MEF-Net}. 
% instead of. In this task, the fused image is usually considered/modelled as a weighted sum of the source images.\cite{MEF-Net}
%The contribution of the source images is relatively equal for a given patch in the fused image.
The \textit{Visible-Infrared image Fusion} (VIF) is a type of the \textit{Multi-Modal image Fusion} (MMF) that aims at fusing the complementary information of infrared and visible modalities to produce robust and informative fused images \cite{IVF_Survey}.  Infrared images provide more intensity information, while visible images offer more texture and gradient information. %Infrared images have more intensity information while visible images have more texture gradient information.
The \textit{Multi-Focus image Fusion} (MFF) aims at generating an all-in-focus image from a series of partially focused images \cite{MFF_Survey}. A patch of multi-focus fused image typically corresponds to only one source image. %a patch in a multi-focus fused image is likely to refer to only one source image.
%修改为，我们认为MEF和VIF任务都是较为平衡的融合任务，而MFF为极端不平衡的，趋向于两极化选择的任务。
%Therefore, we consider that the MEF and VIF tasks are relatively balanced fusion tasks, while MFF is an extremely unbalanced task that tends towards polarized choices. 
Consequently, it can be observed that the MEF and IVF tasks involve relatively balanced fusion, while MFF is an extremely unbalanced task that tends to exhibit polarized choices. To be compatible with these tasks, it is necessary to learn diverse fusion mechanism.
%we consider that MEF is well-balanced fusion, and the fused image can be considered as a weighted sum of the source images. VIF is unbalanced fusion as the intensity information and gradient information are mainly taken from different modalities. MFF is extremely unbalanced due to the bipolar selections.
%Many task-specific fusion methods have been developed in the early days of deep learning. 
%In the early days of deep learning, numerous task-specific fusion methods have emerged. For instance, \cite{DenseFuse,Deepfuse,CNN} tackle their respective task by leveraging depth features. Many GAN-based \cite{MEF-GAN,TarDAL} and Transformer-based \cite{YDTR,DATFuse,CDDFusion,TransMEF,UTUFuse-Net} methods have been proposed in terms of network structure. Furthermore, High-level tasks \cite{SeAFusion,MoE-Fusion} are also introduced to guide the fusion of images. Feature decomposition \cite{DIDFuse,AUIF} for high-low frequency has also gained significant attention as a research direction. 
%\cite{MEF-GAN,TarDAL} generates fused images by generating adversarial. \cite{DIDFuse,AUIF} guides the extraction of complementary information by decomposing the deep features into low-frequency and high-frequency features.  High-level tasks are introduced to guide the fusion of images \cite{SeAFusion,MoE-Fusion}.Transformer structures are introduced to address the limitation that CNN networks have only local receptive fields \cite{YDTR,DATFuse,CDDFusion,TransMEF,UTUFuse-Net}.
%DeFusion： decompose the source images into the unique component and the shared common component generalizability integrate the complementary information of multiple source images.
%
% U2Fusion: 1.传统方法有限性和复杂性限制了性能的提升。2.端到端模型专门设计GT或无监督指标解决单个任务，多个任务的普遍GT或无参考度量不存在，构成了模型统一学习的主要障碍
%     2. 不同融合任务有相似的目标，即整合多源图像的重要和互补信息。但在不同任务中，需要整合的重要信息变化很大，任务特定方法不适用。由于神经网络具有较强的特征表示能力，统一表示不同信息，使统一融合框架成为可能。3. 统一模型存在相互促进的情况。
% IFCNN：但目前的模型缺乏泛化能力，只能在一种特定类型的图像上表现良好。然而，这个问题将给我们开发基于CNN的算法带来巨大的困难，以融合在没有地面真实图像的情况下的图像（如红外视觉图像和CT-MR图像）
% PMGI：大多数方法只适用于特定的融合任务，而不是泛化的。从图像融合的本质出发，设计一种通用的方法具有重要意义。将融合问题转化为梯度和强度信息的维护。定义了多个图像融合任务的统一形式的损失函数
% SDNet、SwinFusion：直接介绍任务特定融合和统一融合，没有阐述原因。
%需求：1. 任务特定模型只适用于特定的融合任务，不具备泛化能力。
    % 2.部分任务如VIF没有Ground Turth，开发算法困难，需要从其他融合任务泛化过来。（来自IFCNN，早期适用，现在感觉不适用了）
% 由于什么什么的需求，general image fusion这种使用统一框架实现多种融合任务的方法变得越来越重要（单任务无法满足这一要求）
% 一些方法（IFCNN）通过学习一种融合任务，并将其泛化到其他场景，实现单一模型对不同场景的融合；
% 一些方法（U2Fusion,DeFusion）强调对不同场景融合任务共性的学习，......

With the rapid development of deep learning techniques, image fusion has achieved great progress in recent years~\cite{DenseFuse,Deepfuse,U2Fusion}, while most existing methods~\cite{MEF-Net,DDFM,CDDFusion} focus on single image fusion scenario alone. 
Task-specific methods~\cite{MEF-Net,YDTR} often employ task-specific strategies such as designing complex task-biased networks or utilizing task-specific fusion loss functions, resulting in the weak generalization to other tasks~\cite{U2Fusion}.
%weak generalization to other tasks~\cite{U2Fusion}. 
%Although these approaches have demonstrated efficacy within their intended tasks, they generally exhibit limited generalization capabilities when applied to other fusion tasks~\cite{U2Fusion}.
%, resulting in the weak generalization to other tasks~\cite{U2Fusion}. often employ task-specific strategies such as designing complex task-biased networks or utilizing task-specific fusion loss functions
Considering that different fusion tasks have similar objectives, \ie, integrating complementary information from multiple source images, some recently proposed approaches~\cite{IFCNN,U2Fusion,DeFusion} attempted to conduct various fusion tasks using a unified model, forming general image fusion.
These methods, however, are either enmeshed in dominant-task bias~\cite{IFCNN} or multi-task commonality~\cite{U2Fusion,DeFusion} at the expense of individuality, leading to unsatisfactory performance. 
This motivates us to explore a more compatible fusion paradigm that is adaptively and dynamically compatible with different fusion scenarios. 

% many general image fusion methods~\cite{IFCNN,U2Fusion,DeFusion} have been proposed due to those tasks sharing the essence of image fusion.
% These methods accentuate the commonalities among various fusion tasks and achieve excellent performance. 
% These methods bring out the commonalities of different fusion tasks to solve each task.
%\cite{IFCNN} uses MFF supervised training network to learn the extraction of complementary information, which can be generalized to other tasks by simple feature selection. \cite{FusionDN,U2Fusion} performs the information quantity and quality of the source image through the evaluation to determine the degree of feature preservation in different source images.\cite{PMGI} unifies the image fusion problem into the problem of maintaining the texture and intensity ratio of the source images. 
%However, the existing general image fusion is limited by the network's insufficient representation capability to accurately perceive task-relevant fusion rules and dynamically customize the fusion scheme of samples according to the task. This impacts the performance of the model on a single task.
% However, most of these methods 
% However, most existing general image fusion approaches are hindered by the limited representation capability of the networks. As a result, they may struggle to accurately comprehend task-specific fusion rules and dynamically customize fusion schemes for different samples based on certain tasks. This limitation has an impact on the model's performance on a individual task.


%(11.4)为了解决上述问题，我们提出了任务定制的MoA方法。首先，我们使用一个显式的任务定制特征选择模块来处理多源特征。具有任务特定的门控网络的MoE结构可以定制样本的融合规则通过动态的方式。具体来说，任务特定的门控网络通过改变Mixture of shared Experts的分布，学习了特定任务的融合规律。如图1(b)的实验结果所示，不同任务的Mixture of shared Experts的分布具有差异，这一定程度上证实了任务间融合规则的差异确实存在。同时，方差的变化规律也与融合规则的平衡性变化一致。除此之外，我们设计了一个互补特征约束，要求定制特征选择模块评估多源特征在融合特征的百分比参与度。这个约束一方面防止特征跳出解空间，另一方面提供了显式的物理意义。






%为了解决上述问题，我们提出了任务定制的MoA方法。首先，我们使用一个显式的任务定制特征选择模块来处理多源特征。具有任务特定的门控网络的MoE结构可以定制样本的融合规则通过动态的方式。具体来说，任务特定的门控网络通过改变Mixture of shared Experts的分布，学习了特定任务的融合规律。如图1(b)的实验结果所示，不同任务的Mixture of shared Experts的分布具有差异，这一定程度上证实了任务间融合规则的差异确实存在。同时，方差的变化规律也与融合规则的平衡性变化一致。除此之外，我们设计了一个互补特征约束，要求定制特征选择模块评估多源特征在融合特征的百分比参与度。这个约束一方面防止特征跳出解空间，另一方面提供了显式的物理意义。


% \textcolor{red}{Different from existing methods, we first introduce parameter-efficient tuning for multiple image fusion tasks.}
% Our model consists of multiple transformer encoder branches, adapters, and routing networks. The encoders extract features of each source image separately by using a frozen pre-trained foundation model. We borrow the insight from the mixture of experts (MoE), taking each expert as an adapter.
% The task-specific routing networks customize these adapters to fuse task-specific information from different sources, \textcolor{red}{performing visual feature prompt fusion in an adaptive manner}.
% These adapters are shared across different tasks and constrained by a complementary loss, ensuring compatibility with different tasks while complementarity for different sources.
% Extensive experiments demonstrate that TC-MoA outperforms the competing approaches in learning commonalities while retaining compatibility for general image fusion (multi-modal, multi-exposure, and multi-focus), showing superior fusion performance qualitatively and quantitatively.
% Our code will be released for potential broader applications.


% (11.5)
% 为不同任务定制了一个Task-Customized Prompt来指导模型融合
% 不同任务的特定专家生成了一种Apdaters选择分布
% 模型包含任务特定的Routers 和任务共享的 Adapters
%we propose a novel unified image fusion framework, named TC-MoA, which can dynamically adapt to and accommodate various fusion tasks ,thereby breaking through the performance bottleneck of multi-task unified learning. We borrow the insight from the mixture of experts (MoE), and introduce the shared-adapters bank and task-specific routers' bank into our framework. Adapters memorizing different fusion patterns, while routers generate prompt for fusion by customizing a task-biased mixture of adapters with for the current sample. The prompt value, which represents the estimate of the proportion of important information contained in each source, is also referred to as the dominance intensity, indicating the level of dominance a particular source possesses. To guide the learning of dominant intensity of multi-source, we design a complementary loss.


To handle this challenge, inspired by the impressive representation capability of pre-trained foundation models, we introduce the foundation model as a fixed encoder to extract complementary features for multi-source images.
Different from most existing methods, we borrow insight from the mixture of experts (MoE)~\cite{MoE,MMoE}, taking each expert as an efficient tuning adapter to perform adaptive visual feature prompt fusion based on the foundation model.
% These adapters are shared
% across different tasks and constrained by a complementary loss, ensuring compatibility with different tasks while maintaining complementarity for multi-source images.
The task-specific routing networks customize these adapters to generate task-specific fusion prompt for different sources, forming a novel task-customized mixture of adapters (TC-MoA) architecture.
An mutual information regularization is further developed to constrain the prompt, which guarantees complementarity for diverse sources.
It is worth noting that the prompt have significant task bias and dominant intensity gaps. As shown in \cref{fig:introduction}, the prompt of MFF has a greater color difference than VIF and MEF, meaning that feature selection has more bipolarity on dominant intensity bias. Our model effectively perceives the fusion intensity bias among varied fusion tasks in a single model and is therefore compatible with a wider range of fusion tasks.
Extensive experiments verify our superiority over the competing methods in general image fusion, including multi-modal, multi-exposure, and multi-focus fusion.
More importantly, our TC-MoA even shows unprecedented controllability and generalizability for unseen fusion tasks, fully demonstrating our potential in broader scenarios. We summarize our main contributions as follows:
% A complementary loss constrains these adapters across different tasks to extract complementary information.
% % To enhance the compatibility of different fusion tasks, we develop task-customized routers to dynamically combine these adapters, forming a flexible task-customized mixture of adapters (TC-MoA).
% To enhance compatibility, we further developed a flexible task-customized mixture of adapters (TC-MoA) to dynamically combine these adapters for different fusion tasks.
% % we first introduce parameter-efficient tuning to image fusion. Specifically, we freeze all parameters of the pre-trained model except for the TC-MoA module in order to enable cost-effective and swift fine-tuning.
%需要定义loss的正式名字
%1.complementary loss
%2.information regularisation loss function

%prompt的平均主导强度反映了任务在token-level的融合规律。主导强度差反映了任务在source-level的规律。通过tc-moa动态定制prompt，从而间接动态调制融合规则。

% \notsure{The multi-source features are processed by task-specific routers and task-shared adapters to generate a task-customized prompt, as shown in \cref{fig:introduction}.
% % Each task-specific router masters respective appetite for adapters, and every shared adapter possesses a mechanism for generating the prompt. 
% % For each token pairs from multi-source features, the router for the present task selects the most suitable adapter for customising the prompt. 
% Each router masters task-biased appetite for adapters to customize suitable mixture of adapters, and every shared adapter possesses a mechanism for generating the prompt. Subsequently, the fusion of multi-source features is guided by prompt. 
% % The prompt is constrained by a information regularisation loss function, which guarantees compatibility with different tasks and complementarity for diverse sources. 
% The prompt is constrained by a information regularisation loss function, which guarantees complementarity for diverse sources. Thus the prompt represents the estimated value of feature importance for each source image. From this perspective we demonstrate that tasks have different fusion schemes, as shown in \cref{fig:introduction}. Specifically, the prompt for the MFF has a greater colour difference than VIF and MEF, meaning that feature selection has more bipolarity at the patch-level.% i.e., the vast majority of features come from the dominant source.
% %Following this, the fusion layer integrates the fusion feature from  multiple sources with Task-Customized prompt serving as conditions., guiding the fusion of multi-source features. 
% } 
% %Task-customized routers have different appetite for adapters. This phenomenon is demonstrated in  \cref{fig:introduction},  provening by the distances of statistical probability distributions for Adapters. More importantly, the distances of the distributions are also consistent with the degree of balance we analyzed before.
%%%根据prompt的不同颜色值，即 mean value of prompt，图1证明了，任务有不同的融合模式。我们定义信息来源的极化程度为主导强度，即对任务的主导源的依赖程度。
%By averaging the prompt value of dominant source in each patch, 
% \notsure{\cref{fig:introduction} also demonstrates that there are different schemes of tasks. Specifically, the prompt for the MFF task is composed of deep red and deep blue colors, meaning that for a patch of the fused image, the majority of its features come from the dominant source. In contrast, the MEF and VIF tasks retrieve information more uniformly from multi-source images. We define the degree of polarisation of the multi-source as dominant intensity.}






%---------总结-------------三点贡献
% In summary, the contributions of our work include the following three aspects:

% (i)  (ii) fusion dataset, sophisticated loss functions and fusion rules. (iii) The pro￾posed DeFusion is trained only with the COCO dataset and can be used as a unified and versatile framework for various image fusion tasks without any further fine-tuning or introducing an additional fusion rule. It achieves compa-rable or even better performance compared to the most competitive image fusion methods (including supervised ones) on various types of fusion tasks.

%We propose a novel image fusion method called DeFusion by decomposing the source image based on a self-supervised learning framework.
%We propose a new end-to-end image fusion network,which can realize a variety of image fusion tasks uniformly. The proposed PMGI can fuse infrared and visibleimages, multi-exposure images, medical images, multifocus images and remote sensing images well.
%We propose a dual-branch Transformer-CNN framework for extracting and fusing global and local features,which better reflects the distinct modality-specific and modality-shared features.




%We design a specific loss function, which is applicable to almost all image fusion tasks and can achieve expected results by adjusting the weight of each loss item.
%We refine the CNN and Transformer blocks for a better adaptation to the MMIF task. Specifically, we are the first to utilize the INN blocks for lossless information transmission and the LT blocks for trading-off fusion quality and computational cost.
%We design a pretext task, called CUD, for image fusion, which does not rely on the existing supervised image 
%The prompt is constrained by a complementary loss, which guarantees compatibility with different tasks and complementarity for diverse sources

%1 TC-MoA + Parameter-Efficient Fine-Tuning
%1. we propose the first parameter-efficient fine-tuning method for general image fusion which is based on the TC-MoA module to jointly and adaptively prompting various fusion tasks.

%2 互补Loss
%2. We design a complementary loss, which guarantees compatibility with different tasks and complementarity for diverse sources explicitly.

%3 模型扩展性等等
%3. TC-MoA module is plug-and-play for all ViT(Vision Transformer)-based pre-trained models, supports arbitrary size inputs and colour outputs, and is highly scalable and generalisable.


\begin{itemize}
\item We propose a unified general image fusion model, providing a new task-customized mixture of adapters (TC-MoA) for adaptive multi-source image fusion
(benefiting from the dynamically aggregating effective information from the respective modalities).
\item We propose a mutual information regularization for each adapter, which allows our model to more accurately identify the dominant intensity of different source images.
% task-general prompt structure with a feature-regularised loss function, which makes the method interpretable, controllable and generalisable.
\item To the best of our knowledge, we for the first time pro-
pose an MoE-based flexible adapter for the foundation model in general image fusion. By only adding 2.7\% of learnable parameters, our model copes with numerous fusion tasks. Extensive experiments demonstrate our superiority against the competing methods, while showing significant controllability and generalizability.
% TC-MoA module is plug-and-play for all ViT(Vision Transformer)-based pre-trained models, supports arbitrary size inputs and colour outputs, and is highly scalable.
% 可控性
\end{itemize}

%旧版
%(主要) 是第一篇克服了通用图像融合性能上限的文章。本文注意到不同任务之间融合规则的差异，基于MMoE的Adapter网络结构，给每个任务提供了个性空间（个人空间），让网络能够自适应地根据样本调整融合策略。同时，不同任务之间的融合规则存在共性，可以相互参考，实现协同进化。
%(次要) 提出了基于Transformer的模态间的互补结构和损失函数设计。本文通过Pick-and-Refine adapter网络结构和损失函数设计，能够引导网络根据学习目标自适应地融合特征。而且输出的Attention图能够显示地表现出不同模态的信息流向，具备一定的物理意义，具有很好的可解释性。
%(辅助) 端到端的 参数高效的 无监督通用图像融合 微调框架。支持任意尺寸输入和无需上色的端到端的彩色图像融合。




%-------------------------------------------------------------------------


==> sec/2_RelatedWork.tex <==
\section{Related Work}
\label{sec:formatting}

% %This section briefly reviews the representative works of
% deep learning (DL)-based multi-modal image fusion (MMIF)
% approaches, and the Vision Transformer (LT, Restormer) as
% well as INN modules employed in CDDFuse.





%1 General Image Fusion
%IFCNN使用MFF单一任务有监督训练网络来学习互补信息的提取，通过设计不同的融合规则就可以泛化到其他任务。FusionDN、U2Fusion通过对源图像进行信息量和质评估，来决定不同源图像中特征的保留程度。由于多任务统一的损失函数主要包含强度和梯度两个部分，一些方法开始在网络结构上增强强度和梯度信息的提取。PMGI将图像融合问题统一到源图像的纹理和强度比例维护问题中，将网络分为梯度路径和强度路径进行信息提取。swinfuse将长距离依赖引入通用图像融合，通过Swin Transformer结构实现全局信息的提取和跨源图像互补信息的集成。DeFusion通过自监督表示学习，无需数据和损失函数就可以分离图像的共有特征和独特特征实现融合。

\noindent\textbf{Image Fusion.}
Image fusion focuses on generating a fused image containing complementary information from different source images.
% In the early days of deep learning, numerous task-specific fusion methods have emerged. For instance,
% 
Some early methods \cite{DenseFuse,Deepfuse,CNN} tackled their respective task by leveraging CNN. 
Then, GAN-based \cite{MEF-GAN,MFI-WHU} and Transformer-based %\cite{YDTR,DATFuse,CDDFusion,TransMEF,UTUFuse-Net}
methods~\cite{YDTR,TransMEF,UTUFuse-Net} have been proposed to improve the fusion quality.
Furthermore, high-level tasks \cite{%SeAFusion,
TarDAL,MoE-Fusion} are also introduced to guide the fusion of images. Feature decomposition \cite{DIDFuse,AUIF} for high-low frequency has also gained significant attention as a research direction. 
Different from these methods, some most recent methods focus on general image fusion that aims to address multiple fusion tasks in a single model.
% Subsequently, methods of general image fusion have been proposed. 
\citet{IFCNN} performed a supervised training framework for MFF, which was generalized to other tasks by adjusting fusion conditions.
% to master the extraction of complementary information. %, which can be generalised to other tasks by adjusting fusion conditions.
\citet{FusionDN,U2Fusion} appraised the quantity and quality of information from source images or features with the image quality assessment (IQA) to decide the fusion paradigm. %Deciding what proportion of the source image should be learnt 
%PMGI和SwinFusion分别使用
%Since the loss function for multi-task unification mainly contains two components, intensity and gradient, some methods start to enhance the extraction of intensity and gradient information in the network structure. 
%\citet{PMGI} unifies the image fusion problem into the problem of maintaining the texture and intensity ratio of the source image.
%\citet{swinfusion} introduces the long-range dependency into generalised image fusion by means of the Swin Transformer structure. % to achieve global information extraction and integration of complementary information across source images. 
PMGI \cite{PMGI} and SwinFusion \cite{swinfusion} incorporated a unified fusion framework and loss function, and separate model training for individual tasks.
%The PMGI approach employed a CNN while SwinFusion utilized transformer, both separate model training for individual tasks. %and separate model training for individual tasks. 
% PMGI \cite{PMGI} and SwinFusion \cite{swinfusion} incorporate a unified fusion framework and loss function. The PMGI approach employs a CNN structure while SwinFusion utilizes Transformer structure, both ensuring separate model training for individual tasks.
\citet{DeFusion} performed a self-supervised fusion framework to learn fusion commonality while ignoring task-specific individuality. 
In this work, we accommodate diverse fusion tasks by dynamically customizing the mixture of adapters, rather than suffering individuality for cross-task commonality.
% a uniform fusion framework at the expense of individuality.
%accommodate diverse cultures, religions, races, and gender identities, without discrimination or oppression. Protecting individual uniqueness contributes to an inclusive and diverse society, maximizing the potential and creativity of each person.


\noindent\textbf{Parameter-Efficient Fine-Tuning.}
%2 Parameter-Efficient Fine-Tuning(PEFT)
%为了将预训练的大模型高效地适配到各自下游应用任务中，产生了许多PEFT的研究。PEFT主要分为在网络中增加参数的Adapter[Adapter、LoRA、SSF]和在输入中增加参数的Prefix Tuning[Prefix Tuning,Prompt Tuning,VPT]两种形式。在视觉领域，VPT将Prompt Tuning 引入了 ViT结构，在许多视觉任务上获得了不错的性能。AdaptFormer利用Adapter结构对原有特征的Scaling代替了相加，进一步减少参数量的同时保持了不错的性能。SSF认为预训练特征和下游任务特征之间的差距较小，通过输入无关的尺度参数和移位参数对原有特征进行线性变化，就可以泛化到各类下游任务。
To efficiently adapt pre-trained models to the respective downstream application tasks, some \textit{Parameter-Efficient Fine-Tuning} (PEFT) studies have been proposed.
PEFT can be mainly divided into the Adapter \cite{Adapter, LoRA, SSF} and the Prefix Tuning \cite{PrefixTuning, VPT}. 
\citet{VPT} introduced prompt tuning to the ViT structure. \citet{AdaptFormer} proposed a new adapter by scaling the original features instead of summing.
\citet{SSF} bridged the gap between the pre-trained features and the downstream task features by linearly varying the original features. 
In this paper, different from these methods that focus on tuning high-level tasks, we for the first time generalize the powerful foundational model to general image fusion.
% but to generalize it for the general image fusion task.

\noindent\textbf{Mixture of Experts.}
%为了提升网络的参数量，Spase-MoE首先将mixture of experts (MoE) 结构引入深度学习框架。在此基础上，Switch和GLaM将MoE结构和Transformer结构相结合，进一步提升了网络容量的上限。此外MoE还用来解决其他问题。MMoE通过引入multi-gate使用MoE解决了多任务问题。LiMoE使用MoE解决视觉语言多模态基石模型的训练。
\citet{MoE} first proposed the mixture of experts (MoE) to increase model capacity without increasing computational complexity. Based on this, \citet{GShard} and \citet{Switch} integrated MoE with the transformer structure, further pushing the upper limit of network capacity. In addition, MoE has been validated as effective in other challenges. \citet{MMoE,Mod-Squad} tackled the multi-task problem by designing multi-gates MoE. \citet{LIMoE} exploited MoE to train the contrastive learning-based vision-language foundation model. Inspired by this, we take each expert as an adapter, forming a task-customized mixture of adapters for tuning our general image fusion framework.



==> sec/3_Method.tex <==
\begin{figure*}[t]
  \centering
    \includegraphics[width=1\linewidth]{img/修图TC-MoA_1115_Method.pdf}
    \vspace{-1.8em}
    \caption{ An overview of our proposed TC-MoA method. Our approach gradually modulates the fusion results by inserting TC-MoA into the frozen ViT backbone. TC-MoA generates task-specific prompt through a task-specific router bank and an shared adapter bank. The fusion layer utilizes prompt as scale and source-specific embeddings as biases to obtain fusion images.}
    
    \label{fig:method_1}
    \vspace{-1em}
\end{figure*}
% 方法写简要介绍流程，介绍后面的定义	
% 定义融合问题一句话
% 我们的方法 通过在冻结的ViT backbone中插入TC-MoA来逐渐地调制融合结果, TC-MoA 通过一个router bank，一个adapter bank来生成任务特定的prompts。融合层以prompts作为放缩，源特定的 embedding作为偏置来获得融合结果。 






\section{Method}
% %In this section, we first introduce the workflow of
% CDDFuse and the detailed structure of each module. For
% simplicity, we denote low-frequency long-range features as
% the base features and high-frequency local features as the
% detail features in the following discussion.

% In this section, we first introduce the self-supervised learning pipeline for image
% fusion in Section 3.1. Next, we elaborate on a carefully designed pretext task
% (i.e., CUD) for self-supervised image decomposition and fusion in Section 3.2.
% Finally, the implementation details are presented in Section 3.3.

% In this paper, we propose a dynamic image fusion framework with a multi-modal gated mixture of local-to-global
% experts, termed MoE-Fusion. In Fig. 2, MoE-Fusion contains two encoders, a Mixture of Local Experts, a Mixture
% of Global Experts, and the auxiliary network.

\subsection{Overview}
% Our CDDFuse contains four modules, i.e., a dual-branch
% encoder for feature extraction and decomposition, a decoder for reconstructing original images (in training stage
% I) or generating fusion images (in training stage II), and the
% base/detail fusion layer to fuse the different frequency features, respectively. The detailed workflow is illustrated in
% Fig 2. Note that CDDFuse is a generic multi-modal image
% fusion network, and we only take the IVF task as an example
% to explain the working of CDDFuse.
%…------提取特征相关事宜-------
%简要介绍流程，介绍后面需要的一些变量的定义，
In this paper, we propose a task-customized mixture of adapters for general image fusion, which is a novel parameter-efficient fine-tuning method to jointly and adaptively prompt various fusion tasks.
% 定义什么是融合问题
% Given a pair of source images ... 
% 给定一对源图像XY, 网络通过聚合不同源的互补信息，得到融合图像O，使其具备源图像尽可能多的重要信息。我们将源图像输入ViT网络，经过Patch Embedding得到源图像的token特征。每个TC-MoA包含一个任务特定的router bank和一个任务共享的adapter bank和一个融合层。
% Given a pair of source images XY, the network integrates complementary information from different sources to obtain the fused image O, which retains  important information from the source images. We input the source images into the ViT network and obtain tokens of the source images through patch embedding layer. Each TC-MoA consists of a task-specific router bank, a task-shared adapter bank, and a fusion layer. 我们的网络通过这些TC-MoA逐步地调制融合结果
%我们定义多源图像在网络中间的特征形状为
Given a pair of source images $ \left \{ (X,Y)  | X,Y\in \mathbb{R}^{H\times W\times 3}\right \}$, the network integrates complementary information from different sources to obtain the fused image $ I_{Fusion} \in \mathbb{R}^{H\times W\times 3} $. As shown in \cref{fig:method_1}, we feed the source images into the ViT network and obtain tokens of the source images through the patch embedding layer. ViT consists of an encoder for feature extraction and a decoder for image reconstruction, both of which are composed of transformer blocks. A TC-MoA is inserted into each $ \tau $ $ (\tau=4)$ transformer blocks in both the encoder and decoder. 
Each TC-MoA consists of a task-specific router bank, a task-shared adapter bank, and a fusion layer. Our network gradually modulates the fusion results through these TC-MoA.

%As shown in \cref{fig:method_1}, the source images $ \left \{ (X,Y)  | X,Y\in \mathbb{R}^{H\times W\times 3}\right \} $ are fed into the frozen backbone and produce fusion image $ I_{Fusion}\in \mathbb{R}^{H\times W\times 3} $. 
%\notsure{Given a pair of source images $ \left \{ (X^{\mathcal{V} },Y^{\mathcal{V} })  \right \} $ for VIF, $\left\{(X^{E},Y^{E})\right\}$ for MEF, $\left\{(X^{F},Y^{F})\right\}$ for MFF. 
%The backbone structure follows the vision transformer (ViT) architecture~\cite{VPT}, and the pre-training parameters are sourced from MAE \cite{MAE}.
%The patch size of image features is set to $ (pHpW)\times C $, where $ pW $ and $ pW $ denote the width and height after reshaping.} %这里放到后面可能更好
%ViT consists of an encoder for feature extraction and a decoder for image reconstruction, both of which are composed of transformer blocks. A TC-MoA is inserted into each $ \tau $ $ (\tau=4)$ transformer block in both the encoder and decoder. 
%In \cref{fig:method_1}, a TC-MoA consists of task-customized routers $ \left \{ G^{\mathcal{V} }, G^{E},G^{F} \right \} $, a set of task-shared adapters $  \left \{ A_{1},\dots,A_{N}  \right \}  $  and a prompting fusion layer $  F $ .
%patch size = 16，image patch化之后的尺寸是pH，pW

\subsection{Task-Customized Mixture of Adapters}
As shown in \cref{fig:method_1} , each TC-MoA consists of a task-specific router bank $ \left \{ G^{\mathcal{V} }, G^{E}, G^{F} \right \} $, a task-shared adapter bank $  \left \{ A_{1},\dots,A_{N}  \right \}  $  and a prompting fusion layer $  \mathcal{F} $ . The TC-MoA includes two main stages: prompt generation and prompt-driven fusion. For ease of expression, we take the VIF as an example, assuming that the input comes from the VIF dataset and uses $G$ to denote $G^V$.

\noindent\textbf{Prompt Generation. }
First, we obtain multi-source features for subsequent processing. The network structure before the $j$-th TC-MoA is defined as $E_{j}(\cdot)$, and the extracted features are defined as $f_{x}$ and $f_{y}$, where $f \in \mathbb{R}^{ pH\times pW \times C} $. We concatenate $ f_{x}   $ and $f_{y}$ as a feature representation of pairs of multi-source tokens. 
This allows tokens from different sources to exchange information in the subsequent network. However, directly computing on the high-dimensional concatenated features will bring amounts of unnecessary parameters. Therefore, we use $L(\cdot)$ to perform feature dimension reduction and obtain the processed multiple-source features $\Phi$ as follows,
%一个TC-MoA block 包括提示的生成和提示驱动的融合两个步骤如下所述。为了简化叙述，以下讨论中默认输入来源于VIF。
%提示的生成。首先，获取多元特征。将第j层TC-MoA之前的网络结构定义为E(),提取的特征定义为f,f。我们首先将f和f拼接起来，形成对一对儿多源ptach的特征表示。以便在之后的网络中，来自不同源的对应位置的ptaches可以相互借鉴来生成提示。拼接之后的特征维度为2C，直接进行后续计算会带来大量的额外参数。所以我们使用L(*)对其进行特征降维。最终我们获得了可被处理的多源特征fai.
%然后，根据fai所属任务的不同，我们从router bank 中选出任务特定的router来定制解决方案，即每对patch的特征应该由adapter bank中的哪些adapters来解决。不同任务的定制方案不同，这可以由图2(b)中的统计结果来证明,即路由对每个adapter的路由次数的构成比(proportion)存在显著差异。具体计算方法如下所示，
%在这之后，我们根据路由的结果，将fai输入adapter bank来获得prompt. 每个adapter可以看作一种融合模式，通过路由组合融合模式来处理当前样本根据任务先验。
%For simplicity in the following discussion the default input is derived from the VIF
%Two phases of prompt generation and prompt-driven fusion. 将第j层TC-MoA之前的由backbone提取的特征定义为E(x),E(y). 
% Prior to the j-th TC-MoA, the backbone extracts features denoted as  $  \left \{ E_{j}(X),E_{j}(Y)  \right \} $, where $  E_{j}(X)\in R^{ pH\times pW \times C} $ . Assuming that the input is $ \left ( X^{\mathcal{V} },Y^{\mathcal{V} } \right )  $ , we calculate the multi-source feature $ \Phi $ as follows,
\begin{equation}
  f_{x}  = E_{j}(X ),f_{y}  = E_{j}(Y )
  \label{eq:GetFeature_1}
\end{equation}
\begin{equation}
  \Phi   = L(Cat(f_{x} ,f_{y} ))
  \label{eq:GetFeature_2}
\end{equation}
where $Cat(\cdot)$ represents the concatenation of features, $ L(\cdot) $ consists of a linear layer and normalization layers. % to reduce dimensionality and integrate features from different sources. 
Next, depending on the task to which $ \Phi $ belongs, we select a task-specific router from the router bank to customize the routing schemes, i.e., which adapters in the adapter bank should be input for each token pair.
%Next, We only input task-customized router $ G(\Phi )^{\mathcal{V} } $ to calculate the adapters that should be routed for each token. The router includes tunable gaussian noise, which follows \cite{MoE}.
\begin{multline}
  G(x) =Softmax(TopK(x\cdot W_{g} + \\
  \mathcal{N}(0,1)\cdot Softplus(x\cdot W_{noise} )))
  \label{eq:G_x}
\end{multline}
where $ TopK(\cdot) $ keeps only the top $  K (K = 2) $ values, setting the rest to $ -\infty $ (after $Softmax(\cdot)$, the value becomes 0 ). $  W_{g}  $ and $ W_{noise}   $ are learnable parameters. The customization routing schemes vary for tasks, as evidenced by the proportion of the number of times that different adapters have been routed in \cref{fig:method_1} (b).
After that 
%calculating the routing schemes
, we weight sum the output from the adapters to obtain the prompt. Each router masters a task-biased appetite for customizing a suitable mixture of adapters, and each adapter generates the prompt. 
%Each adapter can be seen as a fusion paradigm, with the router selecting the fusion paradigms to process the current sample based on the task prior. 
The task-customized multi-source prompt is then calculated as follows,
\begin{equation}
  prompt = GAP(Sigmoid(\sum_{i=1}^{N} G(\Phi )_{i}  \cdot A_{i}(\Phi ))
  \label{eq:prompt}
\end{equation}
where $ GAP(\cdot) $ represents the global average pooling, $ i $ is the index of adapters and $ G(\cdot )_{i} $ is the routing value for the $ i$-th  adapter. The task-customized prompt, denoted as $prompt\in \mathbb{R}^{pH\times pW \times2}$, is composed of $prompt_{x}$ and $prompt_{y}\in \mathbb{R}^{pH\times pW \times1}$ and has a value range of $(0,1)$ . 

\noindent\textbf{Prompt-Driven Fusion.}
The task-customized prompt is constrained by mutual information regularization (MIR), which guarantees complementarity for diverse sources. Thus the prompt can be taken as an evaluation of the proportion of important information in each source. 
By dot-multiplication of multi-source features and prompt, we retain complementary information while removing redundant information. Afterward, considering that the feature representation should contain a source-correlated bias
(e.g. visible or infrared images), we introduce input-independent learnable parameters for each source, i.e., source embedding $ S $. After feature prompting and shifting, we obtain the refined source features $ (h_{x},h_{y}) $ as follows,
% \begin{equation}
%   f_{out}=F (prompt\cdot Cat(E (X )+E (Y^{\mathcal{V} }))+ shift^{\mathcal{V} } )
%   \label{eq:f_out}
% \end{equation}
\begin{equation}
\begin{split}
  h_{x}  =prompt_{x}\cdot f_{x}   + S_{x} \\
 h_{y}  =prompt_{y}\cdot f_{y}   + S_{y} \\
 f_{TC-MoA}=\mathcal{F} (h_{x} +h_{y} )
  \label{eq:prompt_scale}
  \end{split}
\end{equation}
% \begin{equation}
%   f_{TC-MoA}=\mathcal{F} (h_{x} +h_{y} )
%   \label{eq:f_out}
% \end{equation}
% \begin{equation}
%   F(A,B)= Conv((A+ shift_{x}^{\mathcal{\mathcal{V} } }) + (B+ shift_{y}^{\mathcal{\mathcal{V} } }) )
%   \label{eq:f_out}
% \end{equation}
where $S_{x} $ and $S_{y} $ represent the source embeddings of visible and infrared images in VIF respectively.  $\mathcal{F}(\cdot)$ fuses the refined multi-source features using an additive operation and then passes them through a set of convolutional layers. These layers introduce local receptive fields to reduce the checkerboard artifacts and align the solution space of the subsequent transformer blocks. Ultimately, we obtain a fusion feature through the task-customized prompt. To encourage the model to extract important information gradually, the features input into the next transformer block are processed as follows,
\begin{equation}
 \begin{split}
  { f_{x} }' = \lambda _{f}f_{x}  +(1-\lambda _{f}) f_{TC-MoA}, \\
  { f_{y} }' = \lambda _{f}f_{y}  +(1-\lambda _{f}) f_{TC-MoA},
 \end{split}
\end{equation}
where $\lambda_{f}$ is a learnable parameter initialized to 0.5.

\noindent\textbf{Mutual Information Regularization.} 
%为了保证模型自适应地保留重要信息，去除冗余信息。我们约束来自于不同源特征的Prompt尽可能地做出取舍。我们假设特征的信息表示是线性变化的
In order to ensure that the model dynamically retains complementary information while discarding redundant information of multi-source features, we impose regularization constraints on the prompt. Assuming that the information representation of features varies linearly, we define the MIR as follows,
\begin{equation}
    \min {\left | prompt_{x}+prompt_{y}-1  \right |} 
  \label{eq:MIR}
\end{equation}
The MIR allows the model to accurately identify the dominant intensity of different sources, which is positively correlated with the information content of the sources.
% 如图6所示，没有MIR约束的模型的特征，会跳出固定的backbone的表示范围，导致对高频信息表示能力的退化。

\subsection{Task-Customized Loss Function}
%%%%
% 11.15 具体的Loss我觉得可以放在补充材料里面。
%%%%
%This loss function forces the model to assign more weights to dominant source for each token pair . We propose an information regularization for each adapter, which allows our model to more accurately identify the dominant intensity of different source images.

% 除了在网络结构上我们兼容了不同任务的个性，我们还为我们为每个融合任务分别定制了无监督损失函数. 一方面，为了保证每个任务都能自适应地学习互补信息的提取并且保证TC-MoA的正常训练，每个任务的损失函数都添加了Lp和Laux。另一方面，为了能够生成质量良好的融合图像，我们对不同融合任务的融合图像进行了结构信息、强度信息和梯度信息的约束，但约束之间略有不同。具体来说，在VIF中，我们……………………

%\textbf{Task-customized loss function. } 
In addition to accommodating the individuality of different tasks in our network structure, we also customize unsupervised loss functions for each fusion task. We add $ \mathcal{L} _{aux} $ to the loss function of each task to ensure the training of TC-MoA and $ \mathcal{L} _{aux} $ is the auxiliary loss in \cite{MoE} to avoid adapters learning unbalanced. On the other hand, in order to generate high-quality fusion images, we impose constraints on the structural information ($\mathcal{L} _{ssim}$), intensity information ($\mathcal{L} _{Pixel}$) for VIF loss function, and gradient information ($\mathcal{L} _{Grad}$) of the fusion images for different fusion tasks.

For the VIF task, our objective is to retain the most pronounced high-frequency and low-frequency information from the source images in the fused image. Thus, we design the $\mathcal{L} _{MaxPixel}$ and $\mathcal{L} _{MaxGrad}$. To avoid confusing gradients, we retain the sign of the gradient values in all loss functions related to gradient information.
For the MEF task, we consider that the luminance of the fused images should be at an average level with all the gradient information. Thus we design the loss functions for MEF with  $\mathcal{L} _{AvgPixel}$ and ${L} _{MaxGrad}$.  Additionally, we adopt $\mathcal{L} _{mefssim}$~\cite{MEF-Net} which is specially designed for the MEF task, instead of the SSIM loss function.
For the MFF task, we believe that each patch of the fused image should only depend on a single source image with the maximum gradient. This is to prevent the objects' edges in defocused images from being preserved, thereby affecting the quality of the fused image. For this purpose, we select only one of the source images to compute the loss function for each patch in the image, \ie $\mathcal{L} _{MaskPixel}$ and $\mathcal{L} _{MaskGrad}$. Please refer to the supplementary material for details of the loss functions.
% \noindent\textbf{VIF.}
%VIF 在VIF任务中，我们认为源图像的最强的高频信息和最强的低频亮度是是需要保留在融合图像的。所以我们为VIF设计了以下的损失函数,
% In the VIF task, our objective is to retain the most pronounced high-frequency information and low-frequency luminance from the source images in the fused image. Thus, we design the following loss functions for VIF.
% \begin{multline}
%   \mathcal{L} _{V} =\mathcal{L} _{p} +\mathcal{L} _{aux}+ \mathcal{L} _{ssim} + \mathcal{L} _{MaxPixel}+\mathcal{L} _{MaxGrad}
%   \label{eq:G_x}
% \end{multline}
% \begin{equation}
%     \mathcal{L}_{ssim} = \lambda_{1} (1-SSIM(O,X))+\lambda_{2}(1-SSIM(O,Y))
%   \label{eq:MaxPixel}
% \end{equation}
% \begin{equation}
%   \mathcal{L}_{MaxPixel} = \frac{1}{HW}\left \| O-max(X,Y) \right \|_1
%   \label{eq:MaxPixel}
% \end{equation}
% \begin{equation}
%   \mathcal{L}_{MaxGrad} = \frac{1}{HW}\left \|   \nabla O - absmax(\nabla X,\nabla Y) \right \|_1
%   \label{eq:MaxGrad}
% \end{equation}
%where $ \mathcal{L} _{aux} $ is the auxiliary loss in \cite{MoE} to avoid adapters learning unbalancedly. %including load constraints and importance constraints. 
% $ \mathcal{L} _{ssim} $ is loss function base on the structural similarity (SSIM) metric. 
%, and $ \lambda_{1}=\lambda_{2}=0.5 $ in our setting. $ mean(\cdot) $, $ max(\cdot) $ and $ absmax(\cdot) $ denote the element-wise average operation, %maximum selection and maximum absolute value selection respectively. 
%To avoid confusing gradients, we retain the sign of the gradient values in $ \mathcal{L} _{MaxGrad} $. Please refer to the supplementary material for details on the loss function. %It should be noted that we have omitted the hyperparameters in front of each loss function in the formula.
%为了防止梯度混乱，我们保留的梯度的正负号，$ absmax(\cdot) $代表选择绝对值最大的

% \noindent\textbf{MEF.}
% %VIF 在VIF任务中，我们认为融合图像的亮度应该处于一个平均水平，并且使用了MEFNet的MEFloss来约束
% In the MEF task, we consider that the luminance of the fused images should be at an average level with all the gradient information. Thus we design the loss functions for MEF as follows. Additionally, we use MEF-SSIM loss function in \cite{MEF-Net} which is specially designed for the MEF task, instead of the SSIM loss function.
%Furthermore, we use MEFSSIM loss function in \cite{MEF-Net}, which is specially designed for the MEF task, instead of the SSIM loss function. 
%we use the average pixel loss function and the maximum gradient loss function. Furthermore, we use MEFSSIM loss function in \cite{MEF-Net}, which is specially designed for the MEF task, instead of the SSIM loss function. 
% \begin{multline}
%   \mathcal{L} _{E} =\mathcal{L} _{p} +\mathcal{L} _{aux}+ \mathcal{L} _{mefssim} + \mathcal{L} _{AvgPixel}+\mathcal{L} _{MaxGrad}
%   \label{eq:G_x}
% \end{multline}
% \begin{equation}
%   \mathcal{L}_{AvgPixel} = \frac{1}{HW}\left \| O-mean(X,Y) \right \|_1
%   \label{eq:AvgPixel}
% \end{equation}

% \noindent\textbf{MFF.}
% %在MFF任务中，我们认为图像的一个patch应该只学习拥有最大梯度的源图像。这是为了防止失焦的图片的物体边缘被保留,从而影响融合图像质量.
% In the MFF task, we believe that a patch of the image should only learn from the source image with the maximum gradient. This is to prevent the objects' edges in defocused images from being preserved, thereby affecting the quality of the fused image. For this purpose, we select only one of the source images to compute the loss function for each patch in the image. 
% \begin{multline}
%   \mathcal{L} _{F} =\mathcal{L} _{p} +\mathcal{L} _{aux}+ \mathcal{L} _{ssim} + \\
%   \sum_{i=1}^{2} I_{MaxGrad} \circ  (\mathcal{L} _{Pixel}^i+\mathcal{L} _{Grad}^i)
%   \label{eq:G_x}
% \end{multline}
% \begin{multline}
%   \mathcal{L} _{F} =\mathcal{L} _{p} +\mathcal{L} _{aux}+ \mathcal{L} _{ssim} + 
%   \mathcal{L} _{MaskPixel}+\mathcal{L} _{MaskGrad}
%   \label{eq:G_x}
% \end{multline}
%其中I代表mask图,i是源图像(X,Y)的index.当源图像X的patch的最大梯度更大时,mask为1.反之,则为0.
%where $ I $  represents the mask map ($ I\in \mathbb{R}^{pH \times pW \times 1}$), with $ i $ being the index of the source image tuple $ (X,Y) $. When the maximum gradient of the patch in the source image $ X $ is greater, the mask is set to 1. Conversely, it is set to 0.

% \subsection{Window Strategy}
% %\textbf{Details of the network.}
% %受到Swin的启发，我们在冻结的ViT Transformer Block的基础上使用Window Strategy，通过引入可学习的窗口位置偏移。这个策略帮助我们以较低的计算量支持任何尺寸的输入。同时间接获得整张图片的感受野。以往的方法为了降低计算量，只支持固定尺寸的输入，利用额外的预处理和后处理将图片裁剪然后拼接，这会导致棋盘效应。我们通过将图片划分为14*14patch的窗口（为了和预训练时模型处理Token的长度一致），every other block 进行一次Cyclic Shift来获取全局感受野。如图2右侧所示。
% %依据以前的Parameter-Efficient Fine-Tuning(PEFT)的设计，我们把ViT Transformer Block分为X组，每组的第Y个和第Y+1个Block中间插入一个TC-MoA Block。
% %为了进一步增强重建图像的清晰度，我们对输入图像进行一次上采样，在输出的时候下采样。
% We incorporate a window strategy in the frozen ViT transformer blocks by introducing learnable relative position embedding. This strategy not only allows for efficient handling of inputs of different sizes but also captures the complete receptive field of the image while avoiding checkerboard artifacts. Please refer to the supplementary material for details.
%entire receptive field of the image. 这个策略还避免了checkerboard artifacts
%Previous approaches aiming to reduce the computational effort of the transformer only supported fixed-size inputs.They employed additional pre-processing and post-processing steps to crop and stitch the image together, resulting in the checkerboard artifacts. To overcome this, we divide the features into multiple windows of $ 14\times14 $ patch (to maintain consistency with the token length during pre-training). Additionally, we apply cyclic shifts in every other block to acquire a global receptive field.



==> sec/3_finalcopy.tex <==
\section{Final copy}



%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.


%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.


\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/4_Experimental_Results.tex <==
\section{Experiments}
\subsection{Experimental Setting}

%In VIF, LLVIP 数据集有着样本数量多且对齐很好的优点。 We use LLVIP 12025 pairs of 可见光和红外光图像对 as training and 均匀地在3463对测试集图像中选择了 70 samples 来测试.
%In MEF, We use SCIE as training set, MEFB as testing set. SCIE拥有高分辨率的多曝光序列589个。我们从每个序列中选择最欠曝光和最过曝光的作为图像对。MEFB是一个有众多对比方法的benchmark,包含100对测试图像.
%In MFF, We use RealMFF作为主要的训练集, WFI-WHU是辅助的训练集. RealMFF包含710个自然拍摄下的多聚焦图像对,而WFI-WHU包含 120对人造多聚焦图像对.这允许模型学习多种多聚焦模式。 MFFB是一个有众多对比方法的benchmark,包含63对测试图像.
% In VIF, the LLVIP \cite{LLVIP} dataset has the advantage of having a large number of aligned samples.
% We utilize 12025 visible and infrared image pairs for training and randomly selected 70 samples out of 3463 pairs for testing.
% In MEF, we employ the SCIE \cite{SCIE} dataset  for training and MEFB dataset for testing.  The SCIE dataset comprises 589 high-resolution multi-exposure sequences, and we utilize the most underexposed and overexposed images from each sequence to form multi-source image pairs. The MEFB dataset \cite{MEF_Benchmark} is a benchmark, containing 100 pairs of test images.
% In MFF, we use RealMFF \cite{Real-MFF} as the primary training set, with MFI-WHU \cite{MFI-WHU} as a secondary.  RealMFF contains 710 pairs of multi-focus images taken from natural scenes, while MFI-WHU contains 120 pairs of artificial multi-focus images. This allows our model to learn multiple multi-focal patterns. We use dataset of 63 pairs of images in \cite{MFF_DL_Survey} for testing.
\textbf{Datasets.}
We conduct experiments in three image fusion scenarios: visible-infrared, multi-focus, and multi-exposure fusion.
For VIF, we evaluate our model on the LLVIP~\cite{LLVIP} dataset. The training set contains 12025 image pairs, and we randomly select 70 samples out of the test set for evaluation. For MEF, we employ the SCIE \cite{SCIE} dataset (589 pairs) for training and MEFB~\cite{MEF_Benchmark} dataset (100 pairs) for testing, we utilize the most underexposed and overexposed images from sequences in SCIE as inputs.
For MFF, we train our model on the RealMFF~\cite{Real-MFF} and the MFI-WHU~\cite{MFI-WHU} datasets and follow the test setting in MFIF~\cite{MFF_DL_Survey}.
% our primary training set is RealMFF~\cite{Real-MFF} (710 pairs) captured from natural scenes, supplemented by the artificial dataset MFI-WHU~\cite{MFI-WHU} (120 pairs). We follow the test setting in MFIF~\cite{MFF_DL_Survey}.
% For testing purposes, we utilize a dataset of 63 image pairs from \cite{MFF_DL_Survey}.}
\begin{figure}[t]
  \centering
 
    \includegraphics[width=1\linewidth]{img/TC-MoA_vis_VIFv2.pdf}
    \vspace{-1.8em}
    \caption{Qualitative comparisons of various methods in VIF task.}
    \vspace{-1.3em}
    \label{Vis_VIF}
    
\end{figure}


% \textbf{Competing methods. }
% 我们和其他的general image fusion方法对比。IFCNN,FusionDN,PMGI,U2Fusion,DeFusion
\noindent\textbf{Implementation Details.} 
Our experiments are performed on a server with  8 $\times$ NVIDIA RTX A6000 GPUs. Although our model supports inputs of arbitrary size, we ensure that each fusion task receives an equal amount of data per iteration by randomly cropping all samples to a size of $448\times448$.
We employ the pre-trained MAE-large model~\cite{MAE} with GAN loss as our backbone. We train 20 epochs jointly with all the fusion tasks, and the batch size for each fusion task is set to 3. We adopt the AdamW optimizer with the initial learning rate of $1.5\times10^{-4}$. To ensure training stability, we apply the Exponential Moving Average (EMA) to routers and adapters optimization. Each TC-MoA consists of $ N (N=4) $ adapters embedded in different layers, but only the top $ K (K=2) $ adapters are activated.


%Although our model supports inputs of arbitrary size, in order to ensure that each fusion task has the same amount of data in one iteration, we randomly crop all samples to 448×448 size in the preprocessing stage.
%We use MAE-large with GAN loss as the pre-training parameter for the model. During the training process, we perform a 2$ \times $ upsample of the input samples in order to get a better quality of the fused images. We train 20 epochs jointly with all the fusion tasks, and train sequentially in each iteration. The batch size of each fusion task is 3. We adopt the AdamW optimizer with the initial learning rate set to 15e-4. In order to ensure stable training of the network, we use EMA (Exponential Moving Average) for routers, adapters and the relative position embedding. Each TC-MoA has 4 Adapters, and only the top   Adapters are activated. 
%尽管我们的模型支持任意尺寸的输入，但是为了保证每个融合任务在一次训练中的数据量一致，所以我们在预处理阶段将所有样本随机裁剪到 448×448大小。我们使用 large MAE with GAN loss作为模型的预训练参数。在训练过程中，为了让融合图像更加清晰，我们对输入样本进行2×的Upsample.我们用所有融合任务联合训练20个epoch,每次迭代顺序训练三个融合任务. 每个融合任务的 batch size is 3. We adopt the AdamW optimizer with the initial learning rate set to 15e−4 . 为了保持网络的稳定训练，我们对routers,adapters and Window 偏移position 使用EMA的方式训练。每个TC-MoA里面都有4个Adapters,and only  the top 2 Adapters are activated. 


% Implement details. Our experiments are carried out on
% a machine with two NVIDIA GeForce RTX 3090 GPUs.
% The training samples are randomly cropped into 128×128
% patches in the preprocessing stage. The number of epochs
% for training is set to 120 with 40 and 80 epochs in the first
% and second stages, respectively. The batch size is set to 16.
% We adopt the Adam optimizer with the initial learning rate
% set to 10−4
% and decreasing by 0.5 every 20 epochs. For the
% network hyperparameters setting, the number of Restormer
% blocks in SFE is 4, with 8 attention heads and 64 dimensions.
% The dimension of the LT block in BTE is also 64 with 8
% attention heads. The configuration of decoder is the same
% as encoder. As for loss functions Eq. (7) and (10), α1 to α4
% are set to 1, 2, 10, and 2, in order to keep the same order of
% magnitude for each term.

\noindent\textbf{Evaluation Metrics.}
%%%%%%%
% 11.15 提交前修正一遍，把没用到的指标去掉
%%%%%%
%EN、FMI、NMI、PSNR、QNCIE、SCD
%The Image feature-based metrics include Qabf Qp Qg SD 、SF 
%The structural similarity-based metrics include Cvejie’s metric Qc[Qc] Qw Qy Qs[Qs] SSIM MSSSIM MEF-SSIM 
%The Human perception inspired metrics are  Qcb Qcv VIF
%The commonly used metrics for each fusion task are not exactly the same, so we customize a set of metrics for each task. Inspired by \cite{MEF_Survey}, all metrics can be divided into the following four categories. The information theory-based metrics: entropy (EN), peak signal-to-noise ratio (PSNR), normalized MI (NMI), Nonlinear correlation information entropy ( $ Q_{ncie} $), sum of the correlations of differences (SCD), feature mutual information (FMI). The Image feature-based metrics: phase congruency based metric $ Q_{p} $, standard deviation (SD), spatial frequency(SF), gradient-based metric $ Q_{abf}  $and $ Q{g} $. The structural similarity-based metrics: $ Q_{c}  $ \cite{Qc},  $Q_{w} $,  $Q_{y} $ ,  $Q_{s} $ \cite{Qs}, structural similarity (SSIM), multiscale structural similarity (MS-SSIM \cite{MSSSIM}) and MEF-SSIM \cite{MEFSSIM}. The human perception inspired metrics: visual information fidelity (VIF), $ Q_{cb} $ and  $Q_{cv} $. Detailed information on metrics can be found in \cite{IVF_Survey} and  \cite{MFF_Survey}. 
Since the commonly used evaluation metrics for each fusion task are not exactly the same, we customize a set of metrics for each task. Existing metrics can be mainly divided into the following four categories~\cite{MEF_Survey}. $\diamond$ The information theory-based metrics: entropy (EN), peak signal-to-noise ratio (PSNR), mutual information (MI), normalized MI (NMI), Nonlinear correlation information entropy ($ Q_{ncie} $),  feature mutual information (FMI). $\diamond$ The image feature-based metrics: phase congruency-based metric $ Q_{p} $, standard deviation (SD),  gradient-based metric $ Q_{abf} $, and $ Q_{g} $. $\diamond$ The structural similarity-based metrics: $ Q_{c}  $ \cite{Qc},  $Q_{w} $, $Q_{s}$ \cite{Qs}, structural similarity (SSIM), multiscale structural similarity (MS-SSIM \cite{MSSSIM}) and MEF-SSIM \cite{MEFSSIM}. $\diamond$ The human perception inspired metrics: visual information fidelity ($ VIF $), $ Q_{cb} $ and  $Q_{cv} $. Detailed information on metrics can be found in \cite{IVF_Survey} and  \cite{MFF_Survey}.


%sum of the correlations of differences (SCD),spatial frequency(SF),$Q_{y} $ ,
% 信息论相关feature-based：information theory-based metrics: EN、PSMR、MI、NMI、Qncie FMI。
% 特征相关：Qp SD  梯度相关：Qabf Qg 
% 结构相关structural similarity-based：SSIM Qc Qw Qs
% 人类感知human perception inspired：Qcb Qcv VIF
% Comparison of more metrics in the appendix.


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t] \scriptsize
  \centering
   \setlength{\tabcolsep}{2.35pt}
   
   \caption{ Quantitative results of the VIF task in LLVIP dataset. \textbf{Boldface in \textcolor[rgb]{ 1,  0,  0}{red}} and \textbf{boldface in \textcolor[rgb]{ 0,  0,  1}{blue}} show the best and second-best values, respectively. The \underline{underline} represents the best value in the general image fusion methods. }
   \vspace{-1.3em}
    \begin{tabular}{@{}lcccccccc@{}}
    \toprule
    Method & $VIF$ & $ Q_{c} $ & EN & SD & \textbf{$Q_{cv}$↓} & MS-SSIM & FMI & $ Q_{w} $  \\
    \midrule
   Densefuse \cite{Deepfuse} & 0.545 & 0.533 & 6.830 & 9.381 & 817.213 & 0.878 & 0.876 & 0.622 \\
    AUIF \cite{AUIF} & 0.402 & 0.370 & 6.137 & 7.769 & 1087.569 & 0.784 & 0.869 & 0.530 \\
    DIDFuse \cite{DIDFuse} & 0.366 & 0.348 & 5.991 & 7.765 & 897.007 & 0.767 & 0.863 & 0.479 \\
    TarDAL \cite{TarDAL}& 0.550 & 0.562 & {\color[HTML]{0000FF} \textbf{7.347}} & 9.609 & 549.177 & 0.864 & 0.860 & 0.628 \\
    YDTR \cite{YDTR} & 0.486 & 0.524 & 6.638 & 8.810 & 883.333 & 0.835 & 0.876 & 0.614 \\
    RFN-Nest \cite{RFN-Nest} & 0.497 & 0.456 & 7.052 & 9.609 & 857.157 & 0.862 & 0.871 & 0.385 \\
    SwinFuse \cite{Swinfuse}& 0.399 & 0.321 & 5.878 & 7.457 & 1306.652 & 0.734 & 0.870 & 0.425 \\
    UMF-CMGR \cite{UMF_CMGR}& 0.414 & 0.479 & 6.607 & 8.520 & 810.670 & 0.801 & 0.876 & 0.561 \\
    DDFM \cite{DDFM}& 0.588 & 0.561 & 7.069 & 9.696 & 760.006 & 0.908 & 0.878 & 0.663 \\ 
    CDDFuse \cite{CDDFusion}& {\color[HTML]{0000FF} \textbf{0.694}} & {\color[HTML]{FF0000} \textbf{0.645}} & 7.342 & {\color[HTML]{0000FF} \textbf{9.733}} & {\color[HTML]{0000FF} \textbf{495.473}} & 0.933 & {\color[HTML]{0000FF} \textbf{0.883}} & 0.830 \\
    \midrule
    SDNet \cite{SDNet}& 0.527 & 0.575 & 6.897 & 9.318 & 936.389 & 0.878 & 0.872 & 0.749 \\
    IFCNN \cite{IFCNN}& 0.679 & 0.634 & 7.223 & 9.662 & 521.741 & {\color[HTML]{0000FF} \textbf{0.946}} & 0.882 & {\color[HTML]{0000FF} \textbf{0.856}} \\
    U2Fusion \cite{U2Fusion}& 0.503 & 0.492 & 6.647 & 8.789 & 857.455 & 0.878 & 0.870 & 0.695 \\
    DeFusion \cite{DeFusion}& 0.606 & 0.606 & 7.216 & 9.701 & 532.092 & 0.890 & 0.880 & 0.676 \\
    TC-MoA & {\color[HTML]{FF0000} {\ul \textbf{0.726}}} & {\color[HTML]{0000FF} {\ul \textbf{0.637}}} & {\color[HTML]{FF0000} {\ul \textbf{7.428}}} & {\color[HTML]{FF0000} {\ul \textbf{9.805}}} & {\color[HTML]{FF0000} {\ul \textbf{423.773}}} & {\color[HTML]{FF0000} {\ul \textbf{0.949}}} & {\color[HTML]{FF0000} {\ul \textbf{0.886}}} & {\color[HTML]{FF0000} {\ul \textbf{0.858}}}
    \\
    \bottomrule

    \end{tabular}%
  \label{VIF_compare_table}
  \vspace{-1.3em}
\end{table}%s



\subsection{Evaluation on Multi-Modal Fusion}
In this section, we compare our TC-MoA with ten task-specific image fusion methods and four general image fusion methods on the LLVIP dataset.
% : \cite{DenseFuse,AUIF,DIDFuse,TarDAL,YDTR,RFN-Nest,Swinfuse,UMF_CMGR,DDFM,CDDFusion} and general image fusion methods including IFCNN \cite{IFCNN}, SDNet \cite{SDNet}, U2Fusion \cite{U2Fusion} and DeFusion \cite{DeFusion}.

%sum of the correlations of differences (SCD),spatial frequency(SF),$Q_{y} $
\begin{table}[t]\scriptsize
  \centering
\setlength{\tabcolsep}{2.7pt}

\caption{Quantitative results of the MEF task in MEFB \cite{MEF_Benchmark} . }
\vspace{-1.3em}
     \begin{tabular}{@{}lcccccccc@{}}
    \toprule
    Method & Psnr & $ Q_{c} $ & $ Q_{p} $ & $ Q_{g} $ & $ Q_{s} $ & MEF-SSIM & FMI & $ Q_{w} $ \\
    \midrule
    Deepfuse \cite{Deepfuse} & 57.104 & 0.426 & 0.352 & 0.325 & 0.641 & 0.897 & 0.873 & 0.548 \\
    MEF-GAN \cite{MEF-GAN}& 56.947 & 0.309 & 0.124 & 0.246 & 0.487 & 0.772 & 0.846 & 0.300 \\
    MEFNet \cite{MEF-Net} & 56.594 & {\color[HTML]{FF0000} \textbf{0.656}} & {\color[HTML]{0000FF} \textbf{0.595}} & {\color[HTML]{FF0000} \textbf{0.565}} & {\color[HTML]{FF0000} \textbf{0.838}} & 0.914 & {\color[HTML]{FF0000} \textbf{0.890}} & {\color[HTML]{FF0000} \textbf{0.866}} \\
    \midrule
    IFCNN \cite{IFCNN} & {\color[HTML]{0000FF} \textbf{57.195}} & 0.553 & 0.562 & 0.478 & 0.720 & {\color[HTML]{0000FF} \textbf{0.943}} & 0.882 & 0.834 \\
    FusionDN \cite{FusionDN} & 56.977 & 0.500 & 0.504 & 0.434 & 0.672 & 0.924 & 0.877 & 0.776 \\
    PMGI \cite{PMGI} & 57.117 & 0.489 & 0.525 & 0.442 & 0.666 & 0.936 & 0.885 & 0.804 \\
    U2Fusion \cite{U2Fusion} & 57.055 & 0.457 & 0.505 & 0.415 & 0.585 & 0.930 & 0.882 & 0.787 \\
    DeFusion \cite{DeFusion} & 57.131 & 0.539 & 0.378 & 0.376 & 0.751 & 0.902 & 0.877 & 0.733 \\
    TC-MoA & {\color[HTML]{FF0000} {\ul \textbf{57.213}}} & {\color[HTML]{0000FF} {\ul \textbf{0.578}}} & {\color[HTML]{FF0000} {\ul \textbf{0.598}}} & {\color[HTML]{0000FF} {\ul \textbf{0.528}}} & {\color[HTML]{0000FF} {\ul \textbf{0.767}}} & {\color[HTML]{FF0000} {\ul \textbf{0.964}}} & {\color[HTML]{0000FF} {\ul \textbf{0.888}}} & {\color[HTML]{0000FF} {\ul \textbf{0.845}}}
    \\
     \bottomrule
     \end{tabular}%
     \vspace{-2em}
  \label{MEF_compare_table}%
\end{table}%

\noindent\textbf{Quantitative Comparisons}. 
We evaluate the fusion performance on 8 quantitative metrics, as shown in Table~\ref{VIF_compare_table}. Our method outperforms all the general image fusion methods, demonstrating our superior compatibility across multiple fusion tasks.
For most task-specific image fusion methods, TC-MoA also performs remarkable improvements, although these methods deploy complex task-specific designs. 
Specifically, our method achieves a significant advantage in VIF, $Q_{cv}$, and EN metrics correlated to human perception or information theory. This indicates that our fused image conforms more to human visual perception and contains more information from the source images. The results on MS-SSIM, SD, and $Q_{w}$  metrics also explain that our fusion results possess a sufficient amount of structural information and gradient information.
%We achieves the best in 7 metrics and the second best for the other metrics, which proves that our method outperforms not only general image fusion methods but also task-specific methods.

% 如图3所示，我们的方法显然拥有更多细节且符合人类视觉审美。地面的纹理更加清晰，尤其是暗处的树木轮廓很好地表现出来了。行人和背景有更高对比度，车灯的色彩也有更高的饱和度。我们的模型直接可以输出彩色图像，我们也仿照其他方法利用YUV变换给图片上色得到TC-MoA YUV.
\noindent\textbf{Qualitative Comparisons.} %As shown in Figure 3, our method evidently contains more details and aligns with human visual aesthetics. The texture of the ground is also clearer, especially the contours of tree in dark areas are well depicted. There is higher contrast between the subjects and the background, and the colors of the bicycle light are more saturated. Our model can directly output TC-MoA, and we have also utilized YUV transformation, following similar approaches, to colorize images and obtain TC-MoA YUV
As shown in \cref{Vis_VIF}, our model outperforms the competing methods in terms of visual quality. For instance, the contours of the tree in dark areas are well depicted and the background texture is clearer. It is worth noting that our model has the capability to directly generate color images, or we can also follow other approaches to conduct on gray images and colorize the results to obtain TC-MoA$^{YUV}$. 
Compared with the competing methods, our model exhibits higher contrast between foreground and background, and more saturated colors. This comparison demonstrates our model is effective in generating fused images with superior perceptual quality.





%especially the contours of tree in dark areas are well depicted. 
%Additionally, there is higher contrast between the foreground and the background, and the colors of the bicycle light are more saturated. Our model has the capability to directly generate colour images, and we also follows other approaches to colorize images and obtain $ TC-MoA^{YUV}$.

%

\subsection{Evaluation on Multi-Exposure Fusion}

% \begin{table}[t]\scriptsize
%   \centering
% \setlength{\tabcolsep}{2.7pt}
% \caption{Quantitative results of the MEF task in MEFB \cite{MEF_Benchmark} . }
% \vspace{-1.3em}
%      \begin{tabular}{@{}lcccccccc@{}}
%     \toprule
%     Method & Psnr & $ Q_{c} $ & $ Q_{p} $ & $ Q_{g} $ & $ Q_{s} $ & MEF-SSIM & FMI & $ Q_{w} $ \\
%     \midrule
%     Deepfuse \cite{Deepfuse} & 57.104 & 0.426 & 0.352 & 0.325 & 0.641 & 0.897 & 0.873 & 0.548 \\
%     MEF-GAN \cite{MEF-GAN}& 56.947 & 0.309 & 0.124 & 0.246 & 0.487 & 0.772 & 0.846 & 0.300 \\
%     MEFNet \cite{MEF-Net} & 56.594 & {\color[HTML]{FF0000} \textbf{0.656}} & {\color[HTML]{0000FF} \textbf{0.595}} & {\color[HTML]{FF0000} \textbf{0.565}} & {\color[HTML]{FF0000} \textbf{0.838}} & 0.914 & {\color[HTML]{FF0000} \textbf{0.890}} & {\color[HTML]{FF0000} \textbf{0.866}} \\
%     \midrule
%     IFCNN \cite{IFCNN} & {\color[HTML]{0000FF} \textbf{57.195}} & 0.553 & 0.562 & 0.478 & 0.720 & {\color[HTML]{0000FF} \textbf{0.943}} & 0.882 & 0.834 \\
%     FusionDN \cite{FusionDN} & 56.977 & 0.500 & 0.504 & 0.434 & 0.672 & 0.924 & 0.877 & 0.776 \\
%     PMGI \cite{PMGI} & 57.117 & 0.489 & 0.525 & 0.442 & 0.666 & 0.936 & 0.885 & 0.804 \\
%     U2Fusion \cite{U2Fusion} & 57.055 & 0.457 & 0.505 & 0.415 & 0.585 & 0.930 & 0.882 & 0.787 \\
%     DeFusion \cite{DeFusion} & 57.131 & 0.539 & 0.378 & 0.376 & 0.751 & 0.902 & 0.877 & 0.733 \\
%     TC-MoA & {\color[HTML]{FF0000} {\ul \textbf{57.213}}} & {\color[HTML]{0000FF} {\ul \textbf{0.578}}} & {\color[HTML]{FF0000} {\ul \textbf{0.598}}} & {\color[HTML]{0000FF} {\ul \textbf{0.528}}} & {\color[HTML]{0000FF} {\ul \textbf{0.767}}} & {\color[HTML]{FF0000} {\ul \textbf{0.964}}} & {\color[HTML]{0000FF} {\ul \textbf{0.888}}} & {\color[HTML]{0000FF} {\ul \textbf{0.845}}}
%     \\
%      \bottomrule
%      \end{tabular}%
%      \vspace{-2.3em}
%   \label{MEF_compare_table}%
% \end{table}%


% \begin{figure}[t]
%   \centering
 
%     \includegraphics[width=1\linewidth]{img/TC-MoAv2_MEF.pdf}
%     \vspace{-2em}
%     \caption{Qualitative comparisons in MEF task.}
% \vspace{-0.3em}
%     \label{Vis_MEF}
% \end{figure}


In this section, we compare TC-MoA with three task-specific MEF methods \ie Deepfuse\cite{Deepfuse}, MEF-GAN\cite{MEF-GAN} and MEF-Net \cite{MEF-Net}, and five general image fusion methods \ie IFCNN \cite{IFCNN}, FusionDN \cite{FusionDN}, PMGI \cite{PMGI}, U2Fusion \cite{U2Fusion}, and DeFusion \cite{DeFusion}.

%我们的方法与优于大多数的general image fusion方法并在五个指标上获得了最好的值。值得注意的是IFCNN是在MFF任务上有监督训练的，而我们的方法是无监督训练的。除此之外，我们的方法没有预测决策图，而是直接生成融合图像。
% 我们的任务在MEF-SSIM指标上获得了优异的结果，这得益于TC-MoA对不同任务的兼容性，我们可以利用任务特定的指标来优化而不用担心任务之间的冲突。最好的MEF-SSIM、PSNR、Qp说明了我们的融合结果具有最好的综合性能在MEF任务上。


\noindent\textbf{Quantitative Comparisons.} 
We employ 8 quantitative metrics to evaluate our model and the competing methods on MEFB, as presented in Table~\ref{MEF_compare_table}.  Our model achieves the SoTA performance in the general image fusion methods and achieves competitive results in task-specific methods. For example, our model significantly improves the MEF-SSIM scores due to the compatibility of TC-MoA with diverse tasks, enabling task-specific optimization while reducing task conflicts. The MEF-SSIM focuses on the structure and contrast distortion of images, and $Q_{p}$  measures the phase congruency of the source and fused images. The highest MEF-SSIM, PSNR, and $Q_{p}$ values indicate our effectiveness in the preservation of structural information, detailed features, and image quality in the fused images.
%pointed out that MEF-SSIM only focuses on some features (structure and contrast distortion) of images 
%Qpintroduced a feature based metric based on image phase congruency. The principal moments of phase congruency are
%adopted to define this metric because they contain the information of
%image salient features like edges and corners. The metric is defined as a
%product of three correlation coefficients
%PSNR代表图像质量好，不失真

%如图4所示，我们的方法在过曝光和欠曝光的区域都保留了最多的纹理细节和颜色信息。具体来说，在过曝光区域，我们很好地保留了太阳周围的云的结构信息。在欠曝光区域，我们是唯一一个能够在保持结构清晰的同时保持颜色信息的正确的方法。例如PMGI和U2Fusion方法中热气球的字体颜色完全错误。这是因为我们的梯度约束带有正负符号，这保证了颜色过渡的正确。实际上，对于每一对多曝光图像，合适的融合亮度没有一个客观的标准，但我们的方法可以通过对Prompt进行调制,使图片的融合变得可控。图中的 TC-MoA Light就是调制Prompt得到的亮度更高的融合结果。具体的调制方式见节XXX.
\noindent\textbf{Qualitative comparisons.} As shown in \cref{Vis_MEF}, our method preserves the most texture details and color in both high and low illumination regions. Specifically, in the high illumination region, our model effectively retains more structural information of the clouds around the sun.  In the low illumination region, the colors of the fonts on the hot air balloon are completely confused in the PMGI and U2Fusion methods. As a comparison, our method maintains detailed information while keeping more accurate color information. In fact, there is no objective standard for the brightness of the fused image for multi-exposure images. To solve this problem, our method makes the fusion of images controllable by modulating the prompt. The image of “TC-MoA Light" shows the result of this modulation. Detailed information about the modulation can be found in \cref{PromptControllability}.




% \begin{figure}[t]
%   \centering
 
%     \includegraphics[width=1\linewidth]{img/TC-MoAv2.pdf}
%     \vspace{-2em}
%     \caption{Qualitative comparisons in MFF task.}
%     \label{Vis_MFF}
   
% \end{figure}


\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{img/TC-MoAv2_MEF.pdf}
    \vspace{-2em}
    \caption{Qualitative comparisons in MEF task.}
\vspace{-1.6em}
    \label{Vis_MEF}
\end{figure}



\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{img/TC-MoAv2.pdf}
    \vspace{-2em}
    \caption{Qualitative comparisons in MFF task.}
    \vspace{-0.8em}
    \label{Vis_MFF}
\end{figure}


\begin{table}[th]\scriptsize
    \centering
  \setlength{\tabcolsep}{2.55pt}

  \caption{Quantitative results of the MFF task.}
   \vspace{-1.3em}
     \begin{tabular}{@{}lcccccccc@{}}
    \toprule
     Method &    NMI & $ Q_{ncie} $ & MI & $ Q_{cb} $ & \textbf{$ Q_{cv} $↓} & MS-SSIM & FMI & $ Q_{w} $ \\
    \midrule
       IFCNN \cite{IFCNN}& {\color[HTML]{0000FF} \textbf{0.847}} & {\color[HTML]{0000FF} \textbf{0.825}} & {\color[HTML]{0000FF} \textbf{6.495}} & {\color[HTML]{0000FF} \textbf{0.691}} & {\color[HTML]{0000FF} \textbf{44.373}} & {\color[HTML]{FF0000} \textbf{0.991}} & {\color[HTML]{FF0000} \textbf{0.881}} & {\color[HTML]{FF0000} \textbf{0.912}} \\
       MFF-GAN \cite{MFI-WHU} & 0.728 & 0.820 & 5.689 & 0.609 & 72.460 & 0.977 & 0.876 & 0.877 \\
    \midrule
    FusionDN \cite{FusionDN}& 0.675 & 0.818 & 5.449 & 0.519 & 178.491 & 0.942 & 0.864 & 0.794 \\
    PMGI \cite{PMGI}& 0.702 & 0.819 & 5.522 & 0.542 & 140.957 & 0.923 & 0.866 & 0.575 \\
    U2Fusion \cite{U2Fusion}& 0.670 & 0.818 & 5.329 & 0.530 & 142.325 & 0.948 & 0.867 & 0.830 \\
    DeFusion \cite{DeFusion}& 0.768 & 0.821 & 5.838 & 0.625 & 83.195 & 0.960 & 0.870 & 0.685 \\
    TC-MoA & {\color[HTML]{FF0000} \textbf{0.875}} & {\color[HTML]{FF0000} \textbf{0.827}} & {\color[HTML]{FF0000} \textbf{6.695}} & {\color[HTML]{FF0000} \textbf{0.718}} & {\color[HTML]{FF0000} \textbf{36.512}} & {\color[HTML]{0000FF} \textbf{0.990}} & {\color[HTML]{0000FF} \textbf{0.881}} & {\color[HTML]{0000FF} \textbf{0.891}}
\\
    \bottomrule
    \end{tabular}%
  \label{MFF_compare_table}%
   \vspace{-2em}
\end{table}%
%This is because our gradient constraints are computed with signed numbers, which ensures that the colour transitions are accurate. For example, the colours of the fonts of the hot air balloon in the PMGI and U2Fusion methods are completely confused. In fact, for each pair of multi-exposure images, there is no objective standard for the brightness of the fused image, but our method makes the fusion of the images controllable by modulating the prompt. The TC-MoA Light in the figure is the result of modulating. See \ref{PromptApplications} for details of the modulation.


\subsection{Evaluation on Multi-Focus Fusion}


% \notsure{In this section, we compare TC-MoA with general image fusion methods \ie IFCNN \cite{IFCNN}, FusionDN \cite{FusionDN}, PMGI \cite{PMGI}, U2Fusion \cite{U2Fusion}, and DeFusion \cite{DeFusion}. }

% \notsure{In this section, we compare TC-MoA with image fusion methods \ie IFCNN \cite{IFCNN}, MFF-GAN \cite{MFF-GAN}, FusionDN \cite{FusionDN}, PMGI \cite{PMGI}, U2Fusion \cite{U2Fusion}, and DeFusion \cite{DeFusion}. }

We compare TC-MoA with two task-specific MFF methods \ie  IFCNN \cite{IFCNN} (supervised on MFF) and MFF-GAN \cite{MFF-GAN}, and four general image fusion methods \ie FusionDN \cite{FusionDN}, PMGI \cite{PMGI}, U2Fusion \cite{U2Fusion}, and DeFusion \cite{DeFusion}. 
% 尽管如此，我们仍然在NMI、MI、Qcb和Qcv指标上显著优于IFCNN。这说明我们的融合结果保留了更多的源图像信息且具有更好的视觉效果。


\noindent\textbf{Quantitative Comparisons.} 
We employ 8 quantitative metrics on the dataset provided in the \cite{MFF_DL_Survey},  as illustrated in Table~\ref{MFF_compare_table}. Our method shows competitive performance compared to most image fusion methods. 
% It is worth mentioning that IFCNN is supervised trained on the MFF task, while our method is unsupervised trained. 
For general image fusion, our model achieves superior performance across all metrics. Additionally, TC-MoA directly generates the fused image without predicting the decision map. Nevertheless, we still significantly outperform IFCNN in NMI, MI, Qcb, and Qcv metrics. This indicates that our fusion results, compared to supervised method, retain more source image details and demonstrate remarkable human visual perception.

% 信息论相关feature-based：information theory-based metrics: EN、PSMR、MI、NMI、Qncie FMI。
% 特征相关：Qp SD  梯度相关：Qabf Qg 
% 结构相关structural similarity-based：SSIM Qc Qw Qs
% 人类感知human perception inspired：Qcb Qcv VIF
% 特别是，他在VIF、Qcv、EN这三个基于人类感知或信息论的指标上获得了压倒性的优势，这说明我们的融合图像更符合人类的视觉感知，包含更多的源图像的信息。MS_SSIM、SD、Qw上的结果也说明了我们的融合结果具备充足的结构信息和梯度信息。


%如图5所示，我们的融合图像拥有和原图最一致的纹理和颜色，并是所有方法里视觉效果最好的。其他方法比如U2Fusion在远焦区域的重建颜色上有所偏差，IFCNN在近焦图像上失真。其他的方法都没办法很好地去除花朵周边的失真，但得益于我们特殊设计的MFF损失函数，我们的花朵视觉效果最好。我们只选择单个源作为融合图像的参考。
\noindent\textbf{Qualitative Comparisons.} 
As depicted in \cref{Vis_MFF}, our fused image exhibits superior consistency in terms of texture and color, surpassing that of the other methods. U2Fusion exhibits color deviations in the far-focus region, while IFCNN distorts the near-focus image. Furthermore, these methods are unable to effectively remove the distortion around the flowers. As a comparison, we introduce an MFF-specific loss, which achieves the most visually appealing results for the flower.





\subsection{Ablation Study}
We conduct ablation studies to verify the effect of our TC-MoA, MIR, and network architecture.
%如表N所示，在VIF和MFF任务上，多任务训练给网络带来了提升，

% \begin{table}[t]\tiny
%     \centering
%   \setlength{\tabcolsep}{1.7pt}
%   \caption{Add caption}
%     \begin{tabular}{@{}lcccccccc@{}}
%     \toprule
%     \multicolumn{9}{c}{\textbf{LLVIP on mulit-modal fusion}} \\
%     {Method} &  {VIF} &  {SCD} &  {Qabf} &  {SSIM} & {MSSSIM} &  {Qp} & {Qcb} &  {Qc} \\
%     \midrule
%     MoA on LLVIP & 0.6678  & 1.3983  & 0.5474  & 0.4134  & 0.8927  & 0.3606  & 0.4723  & 0.6088  \\
%     Mulit-Task without MoA & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.7224 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{1.5290 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.5997 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.4544 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.9491 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.4116 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.4942 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.6357 }} \\
%     TC-MoA on Mulit-Task & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.7258 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1.5343 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.6007 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.4550 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.9494 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.4119 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.4940 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.6365 }} \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%

% \begin{table}[t]\tiny
%     \centering
%   \setlength{\tabcolsep}{1.7pt}
%   \caption{Add caption}
%     \begin{tabular}{@{}lcccccccccc@{}}
%     \toprule
%     \multicolumn{11}{c}{\textbf{LLVIP on mulit-modal fusion}} \\
%     {Method} &  {VIF} &  {SCD} &  {Qabf} &  {SSIM} & {MSSSIM} &  {Qp} & {Qcb} &  {Qc}  & {Qs} &  {Qg}\\
%     \midrule
%     MoA on MEF & 0.6493  & 0.5224  & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.6387 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.4121 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.9625 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.5918 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.4305 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.5774 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.7670 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.5262 }} \\
%     Mulit-Task without MoA & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.6494 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.5396 }} & 0.6362  & 0.4106  & 0.9622  & 0.5899  & 0.4292  & 0.5765  & 0.7651  & 0.5208  \\
%     TC-MoA on Mulit-Task & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.6615 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.5559 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.6449 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.4116 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.9640 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.5980 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.4310 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.5776 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.7667 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.5276 }} \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%







% \begin{table}[t]\tiny
%     \centering
%   \setlength{\tabcolsep}{1.7pt}
%   \caption{Add caption}
%     \begin{tabular}{@{}lcccccccccc@{}}
%     \toprule
%     \multicolumn{11}{c}{\textbf{LLVIP on mulit-modal fusion}} \\
%     {Method} &  {VIF} &  {SCD} &  {Qabf} &  {SSIM} & {MSSSIM} &  {Qp} & {Qcb} &  {Qc}  & {Qs} &  {Qg}\\
%     \midrule
%        MoA on MFF & 0.8938  & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.5267 }} & 0.6529  & 0.6772  & 0.9879  & 0.6720  & 0.7140  & 0.7694  & 0.9232  & 0.6154  \\
%     Mulit-Task without MoA & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.8978 }} & 0.5180  & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.6562 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.6792 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.9894 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.6799 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.7181 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.7742 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.9246 }} & \textcolor[rgb]{ .267,  .447,  .769}{\textbf{0.6227 }} \\
%     TC-MoA on Mulit-Task & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.8979 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.5344 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.6568 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.6794 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.9897 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.6811 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.7184 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.7755 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.9256 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.6234 }} \\
    
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%










%这里要探讨单任务-多任务-TC-MoA多任务的差异
%由表4可知，在六个常见的指标上，多任务训练的模型整体上优于单任务训练的模型。但是，在MEF任务上,这种规律是相反的，即单任务训练的模型优于多任务。我们认为这反映了多任务模型的多个任务之间产生了竞争，MEF任务的性能被牺牲了。而使用了TC-MoA block的模型在所有任务上都拥有更好的性能。这表明任务之间的竞争被弱化了，每个任务的个性得到了更好的保留。 Single-task vs multi-task. are exhibited
\noindent\textbf{TC-MoA.} 
To verify the effectiveness of TC-MoA, we remove it from our framework. As shown in the first and second rows of Table~\ref{Ablation_single_mulit_Lp}, 
the models trained by multi-task training outperform those trained for a single task, based on 5 commonly used metrics. Interestingly though, this rule reverses in the case of MEF, indicating that inter-task competition occurs for models trained directly with multiple tasks. Comparatively, the model incorporating the TC-MoA improves the performance across all metrics, suggesting that TC-MoA is dynamically compatible with different tasks.
%However, on the MEF task, the regularity is reversed, i.e. the single-task trained model outperforms the multi-task.  We believe that this reflects the competition between the multiple tasks, and the performance of the MEF task is sacrificed. In contrast, the model with the TC-MoA has better performance on all tasks. This suggests that the competition between tasks is reduced and the individuality of each task is better preserved.
%这里要探讨是否使用Lp的差异
%在表4中我们还可以观察到如果模型没有使用互补约束损失函数Lp，绝大多数指标的数值就会大幅下降。尽管VIF在MEF和MFF任务上上升，模型的输出是糟糕的，如图X所示. 我们认为模型缺少了 $L_{p}$ ,prompt的剧烈变化，导致图片的特征跳出冻结的MAE参数的接受范围，最终造成输出的崩溃。

\noindent\textbf{MIR.}
To verify the effectiveness of MIR, we removed MIR from our framework. 
As shown in the last two rows of Table~\ref{Ablation_single_mulit_Lp}, all the evaluation metrics significantly decreased without MIR, indicating the effectiveness of MIR in learning complementary information from multi-source images. 
% it is also discernible that omitting the MIR leads to a significant decrease in the values of metrics. 
The image of the model without MIR constraint tends to exceed the fixed acceptance range of the backbone representation, resulting in a degradation of the ability to represent high-frequency information. As shown in \cref{Vis_network_design}, the shadow details are missed without MIR.
% This further validates the effectiveness of  
%This can be attributed to the drastic changes in the prompts, which occur in the absence of $\mathcal{L}_{p}$. This causes the features of the image to exceed the acceptance range of the frozen MAE parameter, consequently leading to a crash in the output. 
%Despite the fact that VIF increases on the MEF and MFF tasks, the output of the model is abysmal, as shown in \cref{Vis_network_design}. We consider that prompt changes dramatically without $\mathcal{L}_{p}$, resulting in the features of the images not being able to be constrained inside feasible solution for the frozen MAE parameter. This ultimately leads to a collapse of the output.

% 具体来说，Our backbone is ViT-large, which has 24 transformer blocks in encoder and 8 in decoder.
\begin{figure}[t]
  \centering
    
    \includegraphics[width=1\linewidth]{img/TC-MoA1112.pdf}
    \vspace{-2.1em}
    \caption{Ablation studies about network design on LLVIP dataset.}
    \label{Vis_network_design}
    \vspace{-1.6em}
\end{figure}




\noindent\textbf{Network Architecture.}
%图六中通过对比LLVIP数据集上的输出，证明了一些网络结构设计的必要性。第一，如果把图片分窗口预测，不同窗口之间没有信息交互导致拼合时出现不一致。window strategy 通过窗口的滑动避免了不一致问题。第二，只依靠长距离依赖 from transformer 无法准确地提供周边patch的信息,导致棋盘效应(Checkerboard Artifacts)。So we introduce local sensory fields via convolutional layer. 第三，仅仅依靠梯度绝对值的约束生成图像会导致梯度方向的混淆，所以我们使用带符号的梯度约束。第四，我们的模型性能依赖于冻结的ViT参数，普通的MAE-large只使用MSE约束patch的重建，所以高频表示能力很差。
We explore the effect of four network architectures in our framework. The qualitative results are shown in \cref{Vis_network_design}. 
% The necessity of some network structure design is demonstrated in \cref{Vis_network_design}. 
i) Predicting images in isolated windows neglects the inter-window information exchange, thereby yielding inconsistencies across the entire image. Our method enables the interaction of information across the entire image by shifting windows, thereby maintaining the overall coherence of the image.
ii) The transformers are not able to effectively transmit information to adjacent patches solely based on long-range dependencies, resulting in the occurrence of the fusion image checkerboard effect. 
%lack the precision to deliver information about surrounding patches, ultimately generating checkerboard artifacts. 
To address this, we introduce local receptive fields via convolutional layers to enhance the interaction of local features and alleviate the checkerboard effect between adjacent patches. iii) Using only gradient constraints with absolute values can lead the network to blindly learn the gradients of the image, resulting in the generation of fusion images with incorrect gradient directions, which do not align with human visual perception. The loss function based on the signed value of the gradient avoids confusion in the direction of the gradient. 
iv) The common MAE-large only employs the MSE loss function to regulate patch reconstruction, resulting in a suboptimal high-frequency representation. The MAE-GAN reconstructs images through a generative adversarial loss function, which imposes a stronger constraint on both high-frequency and low-frequency information, resulting in features with excellent representation capabilities in terms of high and low frequencies.




\begin{table}[t]\scriptsize
    \centering
  \setlength{\tabcolsep}{3.4pt}
  
  \caption{Ablation studies on three task. S represents the single-task trained model, while M represents the multi-task training. }
   \vspace{-1em}
    \begin{tabular}{@{}cccccccccc@{}}
    \toprule
   Task & S & M & TC-MoA &  MIR & $ Q_{abf} $ & $ Q_{p} $ & FMI & $ Q_{c} $ & SSIM  \\ 
   \midrule 
     \multicolumn{1}{c|}{} & \checkmark &  &  & \multicolumn{1}{c|}{\checkmark} & 0.5984 & 0.4073 & 0.8857 & 0.6335 & 0.4540 \\
    \multicolumn{1}{c|}{} &  & \checkmark &  & \multicolumn{1}{c|}{\checkmark} & {\color[HTML]{0000FF} \textbf{0.5997}} & {\color[HTML]{0000FF} \textbf{0.4116}} & {\color[HTML]{FF0000} \textbf{0.8862}} & {\color[HTML]{0000FF} \textbf{0.6357}} & {\color[HTML]{0000FF} \textbf{0.4544}} \\
    \multicolumn{1}{c|}{} &  & \checkmark & \checkmark & \multicolumn{1}{c|}{} & 0.5343 & 0.3216 & 0.8798 & 0.5984 & 0.4041 \\
    \multicolumn{1}{c|}{\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}VIF\end{tabular}}} &  & \checkmark & \checkmark & \multicolumn{1}{c|}{\checkmark} & {\color[HTML]{FF0000} \textbf{0.6007}} & {\color[HTML]{FF0000} \textbf{0.4119}} & {\color[HTML]{0000FF} \textbf{0.8862}} & {\color[HTML]{FF0000} \textbf{0.6365}} & {\color[HTML]{FF0000} \textbf{0.4550}} \\  \midrule 
    \multicolumn{1}{c|}{} & \checkmark &  &  & \multicolumn{1}{c|}{\checkmark} & {\color[HTML]{0000FF} \textbf{0.6385}} & {\color[HTML]{0000FF} \textbf{0.5916}} & 0.8875 & 0.5754 & {\color[HTML]{0000FF} \textbf{0.4115}} \\
    \multicolumn{1}{c|}{} &  & \checkmark &  & \multicolumn{1}{c|}{\checkmark} & 0.6362 & 0.5899 & {\color[HTML]{0000FF} \textbf{0.8875}} & {\color[HTML]{0000FF} \textbf{0.5765}} & 0.4106 \\
    \multicolumn{1}{c|}{} &  & \checkmark & \checkmark & \multicolumn{1}{c|}{} & 0.5470 & 0.3627 & 0.8791 & 0.5275 & 0.3419 \\
    \multicolumn{1}{c|}{\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}MEF\end{tabular}}} &  & \checkmark & \checkmark & \multicolumn{1}{c|}{\checkmark} & {\color[HTML]{FF0000} \textbf{0.6449}} & {\color[HTML]{FF0000} \textbf{0.5980}} & {\color[HTML]{FF0000} \textbf{0.8883}} & {\color[HTML]{FF0000} \textbf{0.5776}} & {\color[HTML]{FF0000} \textbf{0.4116}} \\  \midrule 
    \multicolumn{1}{c|}{} & \checkmark &  &  & \multicolumn{1}{c|}{\checkmark} & 0.6517 & 0.6733 & 0.8797 & 0.7702 & 0.6774 \\
    \multicolumn{1}{c|}{} &  & \checkmark &  & \multicolumn{1}{c|}{\checkmark} & {\color[HTML]{0000FF} \textbf{0.6562}} & {\color[HTML]{0000FF} \textbf{0.6799}} & {\color[HTML]{0000FF} \textbf{0.8806}} & {\color[HTML]{0000FF} \textbf{0.7742}} & {\color[HTML]{0000FF} \textbf{0.6792}} \\
    \multicolumn{1}{c|}{} &  & \checkmark & \checkmark & \multicolumn{1}{c|}{} & 0.5534 & 0.4954 & 0.8709 & 0.6570 & 0.5825 \\
    \multicolumn{1}{c|}{\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}MFF\end{tabular}}} &  & \checkmark & \checkmark & \multicolumn{1}{c|}{\checkmark} & {\color[HTML]{FF0000} \textbf{0.6568}} & {\color[HTML]{FF0000} \textbf{0.6811}} & {\color[HTML]{FF0000} \textbf{0.8808}} & {\color[HTML]{FF0000} \textbf{0.7755}} & {\color[HTML]{FF0000} \textbf{0.6794}}

 \\ 


    
    \bottomrule
    \end{tabular}%
  \label{Ablation_single_mulit_Lp}%
  \vspace{-1.6em}
\end{table}%





\subsection{Analysis and Discussion} \label{PromptControllability}


% \begin{table}[t]\scriptsize
%     \centering
%   \setlength{\tabcolsep}{2.9pt}
%   \vspace{-1.3em}
%   \caption{Ablation studies on hyperparameters.}
% \begin{tabular}{cc|ccccccccc}
% \toprule


%  &  & \multicolumn{3}{c}{visible-infrared} & \multicolumn{3}{c}{mulit-exposure} & \multicolumn{3}{c}{mulit-focus} \\
% \multirow{-2}{*}{N} & \multirow{-2}{*}{ $\tau $} & Qabf & VIF & SSIM & Qabf & Qp & MEF-SSIM & Qabf & Qp & SSIM \\  \midrule 
% 1 & 4 & {\color[HTML]{0000FF} \textbf{0.600}} & 0.722 & 0.454 & 0.636 & 0.590 & 0.962 & {\color[HTML]{0000FF} \textbf{0.656}} & 0.680 & 0.679 \\
% 2 & 4 & 0.600 & {\color[HTML]{0000FF} \textbf{0.723}} & {\color[HTML]{FF0000} \textbf{0.455}} & {\color[HTML]{FF0000} \textbf{0.645}} & {\color[HTML]{FF0000} \textbf{0.601}} & {\color[HTML]{0000FF} \textbf{0.964}} & 0.656 & {\color[HTML]{0000FF} \textbf{0.680}} & {\color[HTML]{FF0000} \textbf{0.680}} \\
% 4 & 4 & {\color[HTML]{FF0000} \textbf{0.601}} & {\color[HTML]{FF0000} \textbf{0.726}} & {\color[HTML]{0000FF} \textbf{0.455}} & {\color[HTML]{0000FF} \textbf{0.645}} & {\color[HTML]{0000FF} \textbf{0.598}} & {\color[HTML]{FF0000} \textbf{0.964}} & {\color[HTML]{FF0000} \textbf{0.657}} & {\color[HTML]{FF0000} \textbf{0.681}} & {\color[HTML]{0000FF} \textbf{0.679}} \\
% 8 & 4 & 0.566 & 0.651 & 0.423 & 0.611 & 0.421 & 0.875 & 0.632 & 0.644 & 0.656 \\  \midrule 
% 4 & 2 & 0.448 & {\color[HTML]{0000FF} \textbf{0.608}} & {\color[HTML]{0000FF} \textbf{0.422}} & {\color[HTML]{0000FF} \textbf{0.480}} & {\color[HTML]{0000FF} \textbf{0.287}} & 0.852 & 0.396 & 0.327 & {\color[HTML]{0000FF} \textbf{0.538}} \\
% 4 & 4 & {\color[HTML]{FF0000} \textbf{0.601}} & {\color[HTML]{FF0000} \textbf{0.726}} & {\color[HTML]{FF0000} \textbf{0.455}} & {\color[HTML]{FF0000} \textbf{0.645}} & {\color[HTML]{FF0000} \textbf{0.598}} & {\color[HTML]{FF0000} \textbf{0.964}} & {\color[HTML]{FF0000} \textbf{0.657}} & {\color[HTML]{FF0000} \textbf{0.681}} & {\color[HTML]{FF0000} \textbf{0.679}} \\
% 4 & 8 & {\color[HTML]{0000FF} \textbf{0.459}} & 0.501 & 0.323 & 0.445 & 0.287 & {\color[HTML]{0000FF} \textbf{0.871}} & {\color[HTML]{0000FF} \textbf{0.474}} & {\color[HTML]{0000FF} \textbf{0.405}} & 0.481 \\ \bottomrule
% \end{tabular}
% \label{hyperparameter_table}%
% \end{table}



%


%Firstly, if the images are predicted in windows, there is no information interaction between different windows resulting in inconsistency of the whole image. window strategy avoids the inconsistency problem by shifting the windows. Second, the long-distance dependence from transformer cannot accurately provide the information of the surrounding patches, which leads to checkerboard artifacts. So we introduce local receptive field via convolutional layer. Third, generating images based on the loss function of the absolute value of the gradient leads to confusion about the direction of the gradient, so we use signed gradient constraints.  Fourth, the performance of our model relies on the frozen ViT parameters, and ordinary MAE-large only uses the MSE loss function to constrain the reconstruction of patches, causing a poor high-frequency representation.

%其中，N4$\tua$4代表$N=4$ and $\tua=2$. SSIM 指标在 MEF任务上的结果实际上是MEFSSIM

\begin{figure*}[t]
  \centering
 
    \includegraphics[width=1\linewidth]
    {img/MoA_Scale.pdf}
    \vspace{-2em}
    \caption{ Visualisation of controllability and generalization of our method.  }
    \label{Vis_Scale}
    \vspace{-1.3em}
\end{figure*}

\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{img/TC-MoA_11_16_RoutersMEFVIF.pdf}
    \vspace{-1.6em}
    \caption{Visualisation of different routers on medical images. }
    \label{Vis_diff_router}
    \vspace{-1em}
\end{figure}



% \begin{figure}[t]
%   \centering
 
%     \includegraphics[width=1\linewidth]{img/TC-MoA_11_16_2.pdf}
%     \caption{ The intensity relationship of the prompt in encoder. $Mean(\cdot)$ stands for the average value of $prompt$  for all token pairs where is the dominant source}
%     \label{Vis_diff_dominant}
% \end{figure}

% \subsection{Prompt applications} \label{PromptApplications}
%factors.我们的网络具有很强的可控性。我们将训练好的模型prompt按照公式X进行放缩，可以获得一系列不同程度的图片如X所示。其中$ \mu=0.5 $, $ \alpha $ and $ \beta $是缩放系数。
\noindent\textbf{Prompt Controllability}. 
Employing the formula noted in \cref{prompt_scale}, we manipulate both the scale and shift of the prompt provided to the trained model, where $ \mu=0.5 $ represents the mean, while $ \alpha $ and $ \beta $ denote the scaling and shifting factors, respectively. We conduct the manipulation on some samples and present an example in \cref{Vis_Scale} (a).
%We scale and shift the prompts of the trained model according to the formula \cref{prompt_scale}.  where $ \mu=0.5 $, $ \alpha $ and $ \beta $ are the scaling and shifting factor respectively. Afterwards, we can obtain a series of different fused images as shown in \cref{Vis_Scale} (a). 
\begin{equation}
\begin{split}
  prompt_{x}^{'}  = \mu +\alpha (prompt_{x}-\mu )+\beta  \\
  prompt_{y}^{'}  = \mu +\alpha (prompt_{y}-\mu )-\beta 
  \label{prompt_scale}
  \end{split}
\end{equation}


%可以看到随着beta数值的变化，融合图像会偏向某个源图像。我们可以观察到以下两点。beta代表着融合图像偏向某个源图像的程度。beta的数值越大，越偏向于源图像X，反之，更偏向于Y。这符合我们对prompt的物理意义的假设。对于alpha来说，alpha代表两张图像的选择程度。越大的alpha就越注重源图像的选择。举例来说， $ \beta $ = -0.3的样本是与under-exposure image更相似的。当alpha=1时，融合图像的建筑区域变得明亮了，alpha=3时更加明亮，但云的亮度基本没有变化。这说明通过放缩prompt的比例系数，可以促进模型对不同区域进行选择。
%所以beta可以看作对主导强度偏置的控制
Obviously, as the value of $\beta$ increases, the brightness and texture of the fused image increasingly resemble the source image $ X $, and inversely, the source image $ Y $.  Thus, $ \beta $ can be considered as a shifting of the dominant intensity bias. Moreover, a higher value of $ \alpha $ tends to favor one source image over the other in the image patches, which can be considered as a scaling of the dominant intensity deviation.
% alpha 可以作为主导强度的标准差
For example, outputs with $\beta$ = -0.3 are more similar to the under-exposure image globally. As $ \alpha $ increases from 0 to 3, the building areas of the fused image gradually become brighter, but the brightness of the clouds remains basically unchanged. This suggests that changing the scale factor of the prompt motivates the model to select different regions. Overall, this experiment demonstrates that the prompt is controllable and can be linearly transformed to obtain fuse images in different degrees.
%For instance, outputs where $ \beta $ = -0.3 globally align more with the under-exposed images. As $ \alpha $ progresses from 0 to 3, the constructed areas within the fused image progressively brighten, yet the cloud brightness remains predominantly unchanged. This infers that by modulating the scale factor of the prompt, the model can be directed to select distinct regions. Overall, this experiment verifies that the prompt is controllable and can undergo linear transformations to obtain a spectrum of potential outputs.
%The parameter $ \beta $ can be considered as a modification of the dominant intensity bias. Moreover, a higher value of $ \alpha $ tends to favor one source image over the other in the image patches. For instance, when $ \beta $ = -0.3, the resulting outputs are globally more similar to the under-exposed image. In the range of $ \alpha $ values from 0 to 3, the fused image gradually brightens in the building areas, while the brightness of the clouds remains largely unchanged. This indicates that by adjusting the scale factor of the prompts, the model can be influenced to focus on different regions. Overall, this experiment illustrates that the prompt is controllable and can be linearly transformed to yield a variety of potential outputs.

%The fused image is more similar to the source image $ Y $ than to the source image $ X $.  
%This is consistent with our definition of dominant intensity. 
% This is consistent with our assumptions about the physical meaning of prompt, which represents the normalised proportion of the source image information.  It can also be observed that the larger the value of alpha, the more patches  favours one of the source images. For example, outputs with $ \beta $ = -0.3 is more similar to the under-exposure image globally. As$ \alpha $increases from 0 to 3, the building areas of the fused image gradually become brighter, but the brightness of the clouds remains basically unchanged. This suggests that by deflating the scale factor of the prompt , the model can be motivated to select for different regions. Overall, this experiment demonstrates that prompt is controllable and can be linearly transformed to get a range of potential outputs.




%我们的方法具有很强的泛化性，可以zero shot泛化到融合规则相似的任务上。 具体来说，我们把医学图像融合和锐化任务的样本看作为IVF的样本输入模型，得到alpha=1，shift=0的基础图像，如图7(b) and (c) 所示。但由于没有任何融合规则的先验知识，输出的融合图像是一张欠佳的图像，缺失许多高频和低频的信息。然而，通过对prompt进行放缩处理，我们可以为新任务，找到一个适合的融合规则。
% 注意的是，Quickbird是卫星的名字所以大写
\noindent\textbf{Generalizability.} 
Our method is highly generalizable to tasks with similar fusion rules by zero-shot fusion. Specifically, we take samples from medical image fusion dataset~\cite{AANLIB} and pan-sharpening dataset generated by the Quickbird satellite, which are fused based on VIF's paradigm. We obtain a base fused image with $ \alpha=1 $ and $ \beta=0 $, as shown in \cref{Vis_Scale} (b) and (c). However, without any prior knowledge of these unknown tasks, the output fused image is an under-performing image, missing many high and low-frequency information. 
Interestingly, by manipulating the prompt, we can find a suitable fusion rule for these new tasks, obtaining reasonable fusion results.

%不同 router之间有不同的生成prompt的方案。如图8所示,使用MFF的router得到的图像比VIF要暗，在没有梯度引导的地方。这是因为MFF根据梯度选择要参考的源，而没有梯度信息的地方倾向于不做选择，即平均每个源的信息。与之相对的，VIF倾向于保留最大的强度信息。另一方面，在图下方，MFF倾向于只保留一个源的梯度信息，而VIF两个源的梯度信息都要。除此之外，我们还可以在router的选择上具有可控性。我们可以对不同router的融合策略进行加权，得到更可控的结果。




\noindent\textbf{Routers Controllability.} 
As shown in \cref{Vis_diff_router}, the images generated by the MFF router are darker than VIF in areas without gradient guidance. The MFF selects the reference sources based on gradients, it tends to average the information from sources without gradient guidance. In contrast, the VIF router tends to preserve the maximum intensity information. Moreover, at the bottom of the image, the MFF router tends to preserve the gradient information depending on a single source, while the VIF router preserves the gradient information from both sources. Additionally, by manipulating the combination of different routers, our model copes with controlling the dynamic changing fusion degree, obtaining more controllable results.
%VIF tends to preserve the maximum strength information. Additionally, at the bottom of the figure, MFF tends to retain gradient information from only one source, while VIF retains gradient information from both sources. Moreover, we can have control over the selection of routers. We can weight the fusion strategies of different routers to achieve more controllable results.

%the image obtained using the MFF router is darker than the VIF in areas without gradient guidance. This is because the MFF selects the reference sources based on gradients, and areas without gradient information tend to not make a selection, averaging the information from each source. In contrast, the VIF tends to preserve the maximum intensity information. On the other hand, at the bottom of the image, the MFF tends to preserve the gradient information from only one source, while the VIF preserves the gradient information from both sources. Additionally, we can have control over the selection of routers. By weighting the fusion strategies of different routers, we can obtain more controllable results.





\noindent\textbf{Hyperparameters.} 
We conducted hyperparameters analysis on two aspects: the number of experts ($N$) and the interval between two TC-MoAs ($\tau$). We utilize the ViT-large as our backbone, which consists of 24 transformer blocks in the encoder and 8 in the decoder. If $\tau=4 $, our model contains 8 instances of TC-MoA. We employ two widely-used metrics $Q_{abf}$ and SSIM to inform the selection of hyperparameters. As presented in \cref{Vis_N_tau}, as $ N $ increases, the performance initially increases but eventually declines, with the peak performance detected at $ N=4 $. This suggests that increasing the number of experts does not necessarily enhance the model's performance. Similarly, when $ \tau=4 $, the model demonstrates the best performance across multi-task. Hence, our experiments are conducted under $ N=4 $ and $ \tau=4 $.
%Our backbone is ViT-large, which has 24 transformer blocks in encoder and 8 in decoder, \ie the number of TC-MoA is 8 in our model, if $\tau=4 $. As shown in \cref{hyperparameter_table}, as $ N $ increases, the values of metrics first increase and then decrease, with the best performance at $ N=4 $. This means that the quantity of experts is not necessarily better. Similarly, $\tau $ is supposed to take an appropriate value also.  
% 我们使用两个融合任务常见的指标基于梯度信息的Qabf和基于结构信息的SSIM来指导超参数的选择。类似的，\tau也需要选择一共合适的值，即$ \tau=4 $。因此，在 $ N=4 $并且$ \tau=4 $时，模型在多个任务上有最好的性能。



\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{img/TC-MoA_11.18_3(2).pdf}
    \vspace{-1.3em}
    \caption{Experiments on the hyperparameters.
    % , where N4$\tau$4 represents $N=4$ and $ \tau =4$. The SSIM for MEF is MEFSSIM. 
    }
    \label{Vis_N_tau}
    \vspace{-1.5em}
\end{figure}

==> sec/5_Conclusion.tex <==
\section{Conclusion}

%不同任务可以定制自己的专家组合,来获得prompt指导多源图像的融合.实验证明,所提出的方法在general image fusion方法中取得了SoTA 并且在特定任务方法中取得了有竞争力的结果.我们的方法具有很强的扩展性,可以即插即用到其他的ViT架构的方法. 除此之外更重要的是,我们的方法具有很强的泛化性,可以zero-shot到新任务上.
In this paper, we propose a task-customized mixture of adapters for general image fusion. With the help of TC-MoA, different fusion tasks customize their respective mixture of adapters to obtain prompt guidance for multiple-source image fusion in a unified model.
To ensure compatibility with different tasks while maintaining complementarity for multi-source images, we further propose mutual information regularization to constrain these adapters. 
Experimental results have shown that TC-MoA achieves advanced performance in general image fusion against the competing methods. In addition, TC-MoA demonstrates strong prompt controllability and router controllability to perform flexible manipulation on the fused images.
% showing significant generalizability.

% ies and can be 
% zero-shot applied to new fusion tasks.
